Score-based Pullback Riemannian Geometry: Extracting the Data Manifold Geometry using Anisotropic Flows

Data-driven Riemannian geometry has emerged as a powerful tool for interpretable representation learning, offering improved efficiency in downstream tasks. Moving forward, it is crucial to balance cheap manifold mappings with efficient training algorithms. In this work, we integrate concepts from pullback Riemannian geometry and generative models to propose a framework for data-driven Riemannian geometry that is scalable in both geometry and learning: score-based pullback Riemannian geometry. Focusing on unimodal distributions as a first step, we propose a score-based Riemannian structure with closed-form geodesics that pass through the data probability density. With this structure, we construct a Riemannian autoencoder (RAE) with error bounds for discovering the correct data manifold dimension. This framework can naturally be used with anisotropic normalizing flows by adopting isometry regularization during training. Through numerical experiments on diverse datasets, including image data, we demonstrate that the proposed framework produces high-quality geodesics passing through the data support, reliably estimates the intrinsic dimension of the data manifold, and provides a global chart of the manifold. To the best of our knowledge, this is the first scalable framework for extracting the complete geometry of the data manifold.

==> icml2025/sections/3-data-analysis.tex <==
\section{Riemannian geometry from unimodal probability densities}
\label{sec:unimodal-riemannian geometry}

% \todo{I propose to first define the metric in its most general form from the score, then followed by this section - want to keep this as general as we can for as long as we can.}
We remind the reader that the ultimate goal of data-driven Riemannian geometry on $\Real^\dimInd$ is to construct a Riemannian structure such that geodesics always pass through the support of data probability densities. In this section we will focus on constructing Riemannian geometry that does just that from unimodal densities $\density:\Real^\dimInd\to \Real$ of the form
\begin{equation}
    \density(\Vector) \propto e^{- \stroco(\diffeo(\Vector))},
    \label{eq:stroco-diffeo-density}
\end{equation}
where $\stroco:\Real^\dimInd\to\Real$ is a smooth strongly convex function and $\diffeo:\Real^\dimInd\to\Real^\dimInd$ is a diffeomorphism.
% , e.g., such as the density in \Cref{fig:toy-example}\footnote{Here, $\stroco(\Vector) := 2 \Vector_1^2 + \frac{1}{8}\Vector_2^2$ and $\diffeo(\Vector):= (\Vector_1 - \frac{1}{9} \Vector_2^2, \Vector_2)$.}. 
In particular, we will consider pullback Riemannian structures of the form\footnote{Note that $\nabla \stroco \circ \diffeo$ should be read as $(\nabla \stroco) \circ \diffeo$.}
\begin{equation}
    (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector} := (D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB])_2.
    \label{eq:stroco-diffeo-pullback}
\end{equation}
For proofs of the results below and those of more general statements we refer the reader to \Cref{app:proof-of-basic-setup}.





% What remains to be shown is that such geodesics and other manifold mappings pass through the data support (like in \Cref{fig:toy-example-barycentre,fig:toy-example-geodesic,fig:toy-example-log,fig:toy-example-exp}). 
% \subsection{Manifold mappings}
% \label{sec:manifold-mappings}
The following result, which is a direct application of \citep[Prop.~2.1]{diepeveen2024pulling}, gives us closed-form expressions of several important manifold mappings under $(\cdot,\cdot)^{\nabla \stroco \circ \diffeo}$ if we choose
\begin{equation}
    \stroco(\Vector)=\frac{1}{2} \Vector^{\top} \spdMatrix^{-1} \Vector,
    \label{eq:quadratic-stroco}
\end{equation}
where $\spdMatrix\in \Real^{\dimInd\times \dimInd}$ is symmetric positive definite.

\begin{proposition}
\label{thm:pull-back-mappings}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a function of the form \cref{eq:quadratic-stroco}.

    Then,
    \begin{align}
        &\distance^{\nabla \stroco \circ \diffeo}_{\Real^\dimInd}(\Vector, \VectorB) = \| \spdMatrix^{-1} (\diffeo(\Vector) -  \diffeo(\VectorB))\|_{2},
        \label{eq:thm-distance-remetrized-special-psi} \\
        &\geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t) = \diffeo^{-1}((1 - t)\diffeo(\Vector) + t \diffeo(\VectorB)),
        \label{eq:thm-geodesic-remetrized-special-psi}\\
        &\exp^{\nabla \stroco \circ \diffeo}_\Vector (\tangentVector_\Vector) = \diffeo^{-1}(\diffeo(\Vector) + D_{\Vector} \diffeo[\tangentVector_\Vector]),
        \label{eq:thm-exp-remetrized-special-psi}\\
        &\log^{\nabla \stroco \circ \diffeo}_{\Vector} \VectorB = D_{\diffeo(\Vector)}\diffeo^{-1}[\diffeo(\VectorB) - \diffeo(\Vector)].
        \label{eq:thm-log-remetrized-special-psi}
    \end{align}
\end{proposition}

% Similarly, \cite[Cor.~3.6.1]{diepeveen2024pulling} gives us a closed-form expression of the Riemannian barycentre \citep{karcher1977riemannian} $\Vector^* \in \Real^\dimInd$ of the data set $\{\Vector^\sumIndA\}_{\sumIndA=1}^\dataPointNum$ under $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$
% \begin{equation}
%     \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^{\nabla\stroco\circ\diffeo}(\Vector, \Vector^\sumIndA)^2 \Bigr\} = (\diffeo^{-1} \circ\nabla \stroco^\star)\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \nabla \stroco(\diffeo(\Vector^\sumIndA)) \Bigr),
%     \label{eq:stroco-diffeo-barycentre-formal}
% \end{equation}
% which also simplifies to the barycentre on $(\Real^\dimInd, (\cdot,\cdot)^{\diffeo})$
% \begin{equation}
%     \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^\diffeo(\Vector, \Vector^\sumIndA)^2 \Bigr\} = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr),
%     \label{eq:diffeo-barycentre-formal}
% \end{equation}
% for the special choice of $\stroco$ of the form \cref{eq:quadratic-stroco}.

% Once again, the special case also highlights why we get barycentres in the data support. For instance, in the scenario depicted in \Cref{fig:toy-example-barycentre}, Riemannian barycentre are computed by reversing the effect of the diffeomorphism -- once again transforming the data distribution to a Gaussian -- and then computing the mean of the morphed data points, which is finally mapped back to the original space. Again, this results in a barycentre that lives in the data support.

% \begin{proposition}
% \label{prop:euclidean-diffeo-mean}
%     The barycentre problems \cref{eq:stroco-diffeo-barycentre-formal,eq:diffeo-barycentre-formal} have closed-form solutions given by 
%     \begin{equation}
%         \Vector^* = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr) \quad \text{and}\quad \Vector^* = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr),
%         \label{eq:euclidean-diffeo-mean}
%     \end{equation}
%     which 
% \end{proposition}

% [Add mean as well]

\begin{remark}
\label{rem:stability-manifold-mappings}
    We note that $\ell^2$-stability of geodesics is inherited by \citep[Thm.~3.4]{diepeveen2024pulling}, if we have (approximate) local $\ell^2$-isometry of $\diffeo$ on the data support.
\end{remark}

A direct result of \Cref{thm:pull-back-mappings} is that geodesics will pass through the support of $\density(\Vector)$ from (\ref{eq:stroco-diffeo-density}), in the sense that geodesics pass through regions with higher likelihood than the end points. This can be formalized in the following result.
\begin{theorem}
\label{thm:strong-geodesic-convexity}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a function of the form (\ref{eq:quadratic-stroco}). 
    
    Then, mapping 
    \begin{equation}
        t \mapsto \stroco(\diffeo(\geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t))), \quad t \in [0,1]
        \label{eq:mapping-conexity-theorem}
    \end{equation}
    is strongly convex.
\end{theorem}

The Riemannian structure in \cref{eq:stroco-diffeo-pullback} is related to the Riemannian structure obtained from the \emph{score function}\footnote{Note that the score by itself is not always a diffeomorphism.} $\nabla \log(\density(\cdot)):\Real^\dimInd\to\Real^\dimInd$ if $\diffeo$ is close to a smooth local $\ell^2$-isometry on the data support, i.e., $D_{\Vector} \diffeo$ is an orthogonal operator:
\begin{align}
    & (D_{\Vector} \nabla \log(\density(\cdot))[\tangentVector], D_{\Vector} \nabla \log(\density(\cdot))[\tangentVectorB])_2 \notag \\
    & = (D_{\Vector} \nabla (\stroco \circ \diffeo)[\tangentVector], D_{\Vector} \nabla (\stroco \circ \diffeo)[\tangentVectorB])_2 \notag \\
    & = (D_{\Vector} ((D_{(\cdot)} \diffeo)^{\top} \circ \nabla \stroco \circ \diffeo)[\tangentVector], \notag \\
    & \quad\quad\; D_{\Vector} \left((D_{(\cdot)} \diffeo)^{\top} \circ \nabla \stroco \circ \diffeo\right)[\tangentVectorB])_2 \notag \\
    & \approx \left(D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB]\right)_2 
    = (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector}.
\end{align}
For that reason, we call such an approach to data-driven Riemannian geometry: \emph{score-based pullback Riemannian geometry}. 
% Since we find ourselves in a pullback setting\footnote{This is generally not true when using the score itself for probability densities of the form \cref{eq:stroco-diffeo-density}.}, this allows to construct pullback geometry with closed-form manifold mappings.

% \todo[inline]{Repeat that first of all this structure does what we want it to do as showcased in section 3.1.}


\section{Riemannian autoencoder from unimodal probability densities}
\label{sec:rae}

\Cref{thm:pull-back-mappings} begs the question what $\stroco$ could still be used for. 
% As an application of the proposed score-based pullback Riemannian geometry, we will show in \Cref{sec:rae-guarantees} that under a specific choice of $\stroco$ there is a natural \emph{Riemannian autoencoder} (RAE) \citep{diepeveen2024pulling} with error bounds, which can be used to retrieve the data manifold like in \Cref{fig:toy-example-manifold}.
We note that this case comes down to having a data probability density that is a deformed Gaussian distribution. In the case of a regular (non-deformed) Gaussian, one can compress the data generated by it through projecting them onto a low rank approximation of the covariance matrix such that only the directions with highest variance are taken into account. This is the basic idea behind PCA. In the following we will generalize this idea to the Riemannian setting and observe that this amounts to constructing a \emph{Riemannian autoencoder} (RAE) \citep[Sec.~4]{diepeveen2024pulling}, whose error we can bound by picking the dimension of the autoencoder in a clever way, reminiscent of the classical PCA error bound.

Concretely, we assume that we have a unimodal density of the form \cref{eq:stroco-diffeo-density} with a quadratic strongly convex function $\stroco(\Vector):= \frac{1}{2} \Vector^{\top} \spdMatrix^{-1} \Vector$ for some diagonal matrix $\spdMatrix:= \diag(\spdMatrixDiag_1, \ldots \spdMatrixDiag_\dimInd)$ with positive entries\footnote{Note that this is not restrictive as for a general symmetric positive definite matrix $\spdMatrix$ the eigenvalues can be used as diagonal entries and the orthonormal matrices can be concatenated with the diffeomorphism.}. Next, we define an indexing $\coordIndA_\coordIndC \in [\dimInd]:= \{1, \ldots, \dimInd\}$ for $\coordIndC = 1, \ldots, \dimInd$ such that
\begin{equation}
    \spdMatrixDiag_{\coordIndA_1}\geq \ldots \geq \spdMatrixDiag_{\coordIndA_\dimInd},
\end{equation}
and consider a threshold $\RAErelerror\in [0,1]$. We then consider $\dimInd_\RAErelerror \in [\dimInd]$ defined as the integer that satisfies
\begin{equation}
    \dimInd_\RAErelerror = 
 \min \Bigl\{ \dimInd'\in [\dimInd-1] \; \Bigl\vert \; \sum_{\coordIndC=\dimInd' + 1}^{\dimInd} \spdMatrixDiag_{\coordIndA_\coordIndC}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA} \Bigr\}
\label{eq:dimind-epsilon}
\end{equation}
if $\spdMatrixDiag_{\coordIndA_\dimInd}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA}$ and $\dimInd_\RAErelerror = \dimInd$ otherwise.

% \begin{equation}
%     \dimInd_\RAErelerror := \left\{\begin{matrix}
%  \min \Bigl\{ \dimInd'\in [\dimInd-1] \; \Bigl\vert \; \sum_{\coordIndC=\dimInd' + 1}^{\dimInd} \spdMatrixDiag_{\coordIndA_\coordIndC}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA} \Bigr\}, & \text{if } \spdMatrixDiag_{\coordIndA_\dimInd}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA}, \\
%  \dimInd, & \text{otherwise.} \\
% \end{matrix}\right.  .
% \label{eq:dimind-epsilon}
% \end{equation}


% \todo{we can make a split between epsilon being large and small for the d is zero case.}
Finally, we define the encoder (chart) $\RAEencoder_\RAErelerror:\Real^\dimInd \to \Real^{\dimInd_\RAErelerror}$ 
\begin{multline}
    \RAEencoder_\RAErelerror(\Vector)_\coordIndC := (\log^\diffeo_{\diffeo^{-1}(\mathbf{0})} \Vector, D_{\mathbf{0}}\diffeo^{-1}[\mathbf{e}^{\coordIndA_\coordIndC}])^\diffeo_{\diffeo^{-1}(\mathbf{0})} \\
    \overset{\text{\cref{eq:thm-log-remetrized-special-psi}}}{=} (\diffeo(\Vector), \mathbf{e}^{\coordIndA_\coordIndC})_2, \quad \coordIndC = 1, \ldots, \dimInd_\RAErelerror,
    \label{eq:rae-encoder}
\end{multline}
and define the decoder (inverse chart) $\RAEdecoder_\RAErelerror:\Real^{\dimInd_\RAErelerror} \to \Real^\dimInd$ as
\begin{multline}
    \RAEdecoder_\RAErelerror(\latentVector):= \exp_{\diffeo^{-1}(\mathbf{0})}^\diffeo \Bigl( \sum_{\coordIndC=1}^{\dimInd_\RAErelerror} \latentVector_\coordIndC D_{\mathbf{0}}\diffeo^{-1}[\mathbf{e}^{\coordIndA_\coordIndC}]\Bigr) \\
    \overset{\text{\cref{eq:thm-exp-remetrized-special-psi}}}{=} \diffeo^{-1} \Bigl( \sum_{\coordIndC=1}^{\dimInd_\RAErelerror} \latentVector_\coordIndC \mathbf{e}^{\coordIndA_\coordIndC} \Bigr),
    \label{eq:rae-decoder}
\end{multline}
which generate a Riemannian autoencoder and the set $\RAEdecoder_\RAErelerror(\Real^{\dimInd_\RAErelerror}) \subset \Real^\dimInd$ as an approximate data manifold as in the scenario in \Cref{fig:learned_charts}.

Similarly to classical PCA, this Riemannian autoencoder comes with an error bound on the expected approximation error, which is fully determined by the diffeomorphism’s deviation from isometry around the data manifold. For the proof, we refer the reader to \Cref{app:proof-of-rae-error}.
\begin{theorem}
\label{thm:rae-error}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a quadratic function of the form \cref{eq:quadratic-stroco} with positive definite diagonal matrix $\spdMatrix \in \Real^{\dimInd\times \dimInd}$. Furthermore, let $\density:\Real^\dimInd \to\Real$ be the corresponding probability density of the form \cref{eq:stroco-diffeo-density}. Finally, consider $\RAErelerror\in [0,1]$ and the mappings $\RAEencoder_\RAErelerror:\Real^\dimInd \to \Real^{\dimInd_\RAErelerror}$ and $\RAEdecoder_\RAErelerror:\Real^{\dimInd_\RAErelerror} \to \Real^\dimInd$ in \cref{eq:rae-encoder,eq:rae-decoder} with $\dimInd_\RAErelerror \in [\dimInd]$ as in \cref{eq:dimind-epsilon}.

    Then, 
    \begin{multline}
        \mathbb{E}_{\stoVector \sim \density}[\| D_\RAErelerror(E_\RAErelerror(\stoVector))-  \stoVector\|_2^2] \leq \RAErelerror C_\diffeo \trace (\spdMatrix) + o(\RAErelerror),
        \label{eq:thm-rae-bound}
    \end{multline}
where 
\begin{equation}
    C_\diffeo := \inf_{\RAEboundParam\in [0,\frac{1}{2})}\Bigl\{  \frac{\RAEinvdiffeoRegConstantB \RAEdiffeoRegConstant \RAEinvdiffeoRegConstant}{1 - 2\RAEboundParam} \Bigl(\frac{1 + \RAEboundParam}{1 - 2\RAEboundParam} \Bigr)^{\frac{\dimInd}{2}} \Bigr\} 
\end{equation}
for
\begin{equation}
    \RAEinvdiffeoRegConstantB := \sup_{\Vector\in \Real^{\dimInd}} \{ \| D_{\diffeo(\Vector)} \diffeo^{-1}\|_2^2 e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \},
    \label{eq:RAEinvdiffeoRegConstantB}
\end{equation}
\begin{equation}
    \RAEdiffeoRegConstant := \sup_{\Vector\in \Real^{\dimInd}} \{ |\det (D_{\Vector} \diffeo)| e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \},
    % \label{eq:RAEdiffeoRegConstant}
\end{equation}
and
\begin{equation}
    \RAEinvdiffeoRegConstant := \sup_{\Vector\in \Real^{\dimInd}} \{ |\det (D_{\diffeo(\Vector)} \diffeo^{-1})| e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \}.
    % \label{eq:RAEinvdiffeoRegConstant}
\end{equation}
\end{theorem}

\begin{remark}
\label{rem:interpretability-rae}
    Note that the RAE latent space is interpretable as it is $\ell^2$-isometric to the data manifold if $\diffeo$ is an approximate $\ell^2$-isometry on the data manifold. In other words, latent representations being close by or far away correspond to similar behaviour in data space, which is not the case for a VAE \citep{kingma2013auto}.
\end{remark}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{../results/banana-distribution/rae_manifold.eps}
%     \caption{For $\RAErelerror = 0.1$ we obtain a Riemannian autoencoder with latent dimension $\dimInd_\RAErelerror = 1$, which yields the manifold in orange.}
%     \label{fig:rae-manifold}
% \end{figure}

==> icml2025/sections/4-score-based-learning.tex <==
\section{Learning unimodal probability densities }
\label{sec:adapting-normalizing-flows}
% - Next, we know what type of unimodal distribution is ideal for downstream data processing, we construct a learning problem for it that incorporates the lessons learnt, i.e., we need $\ell^2$-isometry on the data manifold

Naturally, we want to learn probability densities of the form \cref{eq:stroco-diffeo-density}, which can then directly be inserted into the proposed score-based pullback Riemannian geometry framework. In this section we will consider how to adapt normalizing flow (NF) \citep{dinh2017density} training to a setting that is more suitable for our purposes\footnote{We note that the choice for adapting the normalizing flow training scheme rather than using diffusion model training schemes is due to more robust results through the former.}. In particular, we will consider how training a normalizing flow density $\density: \Real^\dimInd\to\Real$ given by 
\begin{equation}
    \density(\Vector):= \frac{1}{C_{\stroco}}e^{- \stroco(\diffeo(\Vector))} |\det(D_{\Vector} \diffeo)|,
    \label{eq:nf-density}
\end{equation}
where $C_{\stroco}>0$ is a normalisation constant that only depends on the strongly convex function $\stroco$, yields our target distribution \cref{eq:stroco-diffeo-density}.

From \Cref{sec:unimodal-riemannian geometry,sec:rae} we have seen that ideally the strongly convex function $\stroco: \Real^{\dimInd} \to \Real$ corresponds to a Gaussian with a parameterised diagonal covariance matrix $\spdMatrix \in \Real^{\dimInd\times \dimInd}$, resulting in more parameters than in standard normalizing flows, whereas the diffeomorphism $\diffeo: \Real^{\dimInd} \to \Real^{\dimInd}$ is regularized to be an isometry. In particular, $\spdMatrix$ ideally allows for learnable anisotropy rather than having a fixed isotropic identity matrix. The main reason is that through anisotropy we can construct a Riemannian autoencoder (RAE), since it is known which dimensions are most important. Moreover, the diffeomorphism should be $\ell^2$-isometric, unlike standard normalizing flows which are typically non-volume preserving, enabling stability (\Cref{rem:stability-manifold-mappings}) and a practically useful and interpretable RAE  (\Cref{thm:rae-error,rem:interpretability-rae}). 

In addition, $\ell^2$-isometry (on the data support) implies volume-preservation, which means that $|\det(D_{\Vector} \diffeo)| \approx 1$ so that the model density (\ref{eq:nf-density}) reduces to the desired form of \cref{eq:stroco-diffeo-density}\footnote{We note that without these constraints (accommodating multimodality) the learned mappings can in principle be used to construct Riemannian geometry and a RAE. However, from the theory discussed in this paper we cannot guarantee stability of manifold mappings nor that the RAE has the right dimension.}. While volume preservation theoretically follows from \(\ell^2\)-isometry, in practice, the flow can only approximate local isometry through optimization. Thus, we found it beneficial to explicitly include a volume-preservation loss, resulting in an adapted normalizing flow loss that enforces both constraints for improved alignment with the desired Riemannian structure.
% - say that our approach will rely on normalizing flow training. However, from the sections above, we have seen that we might want to change some things. The main considerations for constructing useful and stable Riemannian geometry
% -- not just volume preserving diffeomorphisms, but ell2 isometries for stability of geodesics and an interpretable RAE. This is a stronger requirement
% -- anisotropic prior to construct the RAE in the first place

% These observations should be reflected in our parametrisation and subsequent learning scheme. For that consider a data set $(\Vector^\sumIndA)_{\sumIndA=1}^\dataPointNum$, whose density we aim to learn, and let $\mu:= \frac{1}{\dataPointNum}\sum_{\sumIndA=1}^\dataPointNum \Vector^\sumIndA$ be the empirical mean of the data and $\mathbf{Q}\Lambda \mathbf{Q}^\top:= \frac{1}{\dataPointNum-1}\sum_{\sumIndA=1}^\dataPointNum (\Vector^\sumIndA - \mu)  (\Vector^\sumIndA - \mu)^\top$ be the eigendecompisition of the empirical data variance. [Regarding parametrisation, we consider]
% \begin{equation}
%     \stroco_{\networkParams_1} (\Vector):= \frac{1}{2}[] , \quad \diffeo_{\networkParams_2}(\Vector):= \diffeoB \circ   
% \end{equation}

% - parametrisation + initialisation
% -- as we have seen that the we want to train deformed Gaussians, it makes sense to initialize with a linear Gaussian approximation. So we consider invertible neural networks of the form
% -- rational quadratic flows \cite{durkan2019neural}
% -- softplus

% - loss
% -- normalizing flow loss
% -- isometry 
% -- possible loss on trace of A
\vspace{-2em}
\begin{multline}\label{eq:basic_training_objective}
    \mathcal{L}(\networkParams_1, \networkParams_2) := \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[-\log \density_{\networkParams_1, \networkParams_2}(\stoVector)\right] \\
    + \lambda_{\text{vol}} \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[ \log(|\det \bigl( D_{\stoVector} \diffeo_{\networkParams_2} \bigr)|)^2 \right] \\
    +
    \lambda_{\text{iso}} \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[ \|  (D_{\stoVector} \diffeo_{\networkParams_2})^\top D_{\stoVector} \diffeo_{\networkParams_2}  - \mathbf{I}_\dimInd\|_F^2 \right]
    % \lambda_{\text{iso}} \mathbb{E}_{\stoVector \sim \density_{\text{data}}, \eta\sim \mathcal{N}(\mathbf{0}, \mathbf{I})}\left[(\| (D_{\stoVector} \diffeo_{\networkParams_2})^*\eta\|_2^2 - \|\eta\|_2^2)^2\right] 
\end{multline}
where $\lambda_{\text{vol}}, \lambda_{\text{iso}} >0$ and the negative log likelihood term reduces to
\begin{multline}
    % \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[-\log \density_{\networkParams_1, \networkParams_2}(\stoVector)\right] = 
    \frac{1}{2}\mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[\diffeo_{\networkParams_2}(\stoVector)^\top \spdMatrix_{\networkParams_1}^{-1} \diffeo_{\networkParams_2}(\stoVector) \right] + \frac{1}{2} \trace(\log(\spdMatrix_{\networkParams_1})) \\
    - \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[ \log(|\det \bigl( D_{\stoVector} \diffeo_{\networkParams_2} \bigr)|) \right]  + \frac{\dimInd}{2}\log(2\pi),
\end{multline}
where $\spdMatrix_{\networkParams_1}$ is a diagonal matrix and $\diffeo_{\networkParams_2}$ is a normalizing flow with affine coupling layers\footnote{We note that the choice for affine coupling layers rather than using more expressive diffeomorphisms such as rational quadratic flows \cite{durkan2019neural} is due to our need for high regularity for stable manifold mappings (\Cref{rem:stability-manifold-mappings}) and an interpretable RAE (\Cref{rem:interpretability-rae}), which has empirically shown to be more challenging to achieve for more expressive flows as both first-and higher-order derivatives of $\diffeo$ will blow up the error terms in \cref{thm:rae-error}.} \citep{dinh2017density}. For small ambient dimensions, isometry regularization is feasible, but in high dimensions, computing the full Jacobian is impractical. To address this, we use a scalable sliced isometry loss based on Jacobian-vector products, significantly reducing both computational and memory costs while preserving effectiveness. See \cref{app:scalable_isometry_regularisation} for details.




% [remark about initialization]

% \begin{remark}
%     Given the connection between PCA and the RAE discussed in \Cref{sec:rae}, it is reasonable to attempt using PCA for initialization. In particular, given a data set $(\Vector^\sumIndA)_{\sumIndA=1}^\dataPointNum$ this would amount to choosing $\spdMatrix_{\networkParams_1^0}:= \Lambda$ and $\diffeo_{\networkParams_2^0}:= \diffeoB_{\networkParams_2^0}\circ\mathbf{U}^\top \circ (\cdot - \mu)$, where 
%     \begin{equation}
%         \mathbf{U}\Lambda\mathbf{U}^\top = \frac{1}{\dataPointNum-1}\sum_{\sumIndA=1}^\dataPointNum (\Vector^\sumIndA - \mu)  (\Vector^\sumIndA - \mu)^\top
%     \end{equation}
%     is the eigendecomposition of the empirical data variance with $\mu:= \frac{1}{\dataPointNum}\sum_{\sumIndA=1}^\dataPointNum \Vector^\sumIndA$ and $\diffeoB_{\networkParams_2^0}$ is a rational quadratic flow initialized close to identity. However, we note that in practice this might not always yield favorable outcomes. For instance, after applying the rotation matrix $\mathbf{U}$ to image data, using efficient network architectures like CNNs to estimate the rational quadratic flow coefficients becomes less intuitive.
% \end{remark}

==> sections/1-introduction-nf-oriented.tex <==
\section{Introduction}

% Data tend to live near low dimensional non-linear  manifolds as in \Cref{fig:toy-example-manifold}. This manifold assumption \cite{fefferman2016testing} has been popular ever since early work on non-linear dimension reduction \cite{belkin2001laplacian,coifman2006diffusion,roweis2000nonlinear,sammon1969nonlinear,tenenbaum2000global} and can still be observed from more modern machine learning approaches such as diffusion models \cite{song2020score} in recent works such as \cite{sakamoto2024the,pmlr-v235-stanczuk24a}. Actually learning this non-linear structure, or learning a representation, from data has been very successful \cite{demers1992non,kingma2013auto} and remains an active area of research.

Data often reside near low-dimensional non-linear manifolds as illustrated in \Cref{fig:learned_charts}. This manifold assumption \citep{fefferman2016testing} has been popular since the early work on non-linear dimension reduction \citep{belkin2001laplacian,coifman2006diffusion,roweis2000nonlinear,sammon1969nonlinear,tenenbaum2000global}. Learning this non-linear structure, or representation learning, from data has proven to be highly successful \citep{demers1992non,kingma2013auto} and continues to be a recurring theme in modern machine learning approaches and downstream applications \citep{chow2022predicting,gomari2022variational,ternes2022multi,vahdat2020nvae,zhong2021cryodrgn}. 
% \todo{WD: we could cite some high-impact applications such as CryoDRGN.}
% , e.g., with researchers noting that diffusion models \cite{song2020score} often identify the manifold, as evidenced in recent studies \cite{sakamoto2024the,pmlr-v235-stanczuk24a}. 
% Learning this non-linear structure, or representation learning, from data has proven to be highly successful \cite{demers1992non,kingma2013auto} and remains an active area of research.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{../results/banana-distribution/distribution.eps}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% In particular, data-driven Riemannian geometry has recently shown to be a suitable language to learn representations. In this setting, representations are elements living in a geodesic subspace  \cite{arvanitidis2016locally,diepeveen2024pulling,hauberg2012geometric,peltonen2004improved,Scarvelis2023,sorrenson2024learningdistancesdatanormalizing} of the data space under a non-trivial Riemannian structure, i.e., other than the $\ell^2$-inner product on all of space. 
% Besides standard data analysis tasks such as computing distances, means, interpolates and extrapolates of data points, a data-driven Riemannian structure has more potential for representation learning and for downstream problems. For example, many more advanced data processing methods from PCA \cite{fletcher2004principal,diepeveen2023curvature} to flow-matching \cite{chen2023riemannian} have Riemannian counterparts, which have shown fruitful in applications in representation learning with the recent introduction of the curvature corrected Riemannian autoencoder\footnote{Note On top of that gives more interpretatbility [e.g., wrt VAE]]} (CC-RAE) \cite{diepeveen2024pulling} and in downstream tasks such as generation \cite{kapusniak2024metricflowmatchingsmooth}.

Recent advances in data-driven Riemannian geometry have demonstrated its suitability for learning representations.
In this context, these representations are elements residing in a learned geodesic subspace of the data space, governed by a non-trivial Riemannian structure\footnote{rather than the standard $\ell^2$-inner product} across the entire ambient space \citep{arvanitidis2016locally,diepeveen2024pulling,hauberg2012geometric,peltonen2004improved,Scarvelis2023,sorrenson2024learningdistancesdatanormalizing,sun2024geometryaware}. 
Among these contributions, it is worth highlighting that \citet{sorrenson2024learningdistancesdatanormalizing} are the first and only ones so far to use information from the full data distribution obtained though generative models \citep{dinh2017density,song2020score}, even though this seems a natural approach given recent studies such as \citet{sakamoto2024the,pmlr-v235-stanczuk24a}. A possible explanation for the limited use of generative models in constructing Riemannian geometry could lie in challenges regarding \emph{scalability of the manifold mappings}. Indeed, even though the generative models can be trained efficiently, \citet{sorrenson2024learningdistancesdatanormalizing} also mention themselves that it can be numerically challenging to work with their induced Riemannian geometry.

\begin{figure*}[t]
    \centering

    % First row: Projections of RAE for three datasets
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{"results/visualisations/RAE/projections/hemisphere_2_3/riemannian_autoencoder.jpg"}
        \caption{Hemisphere (2,3)}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{"results/visualisations/RAE/projections/sinusoid_1_3/riemannian_autoencoder.jpg"}
        \caption{Sinusoid (1,3)}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{"results/visualisations/RAE/projections/sinusoid_2_3/riemannian_autoencoder.jpg"}
        \caption{Sinusoid (2,3)}
    \end{subfigure}

    \caption{
        Approximate data manifolds learned by the Riemannian autoencoder generated by score-based pullback Riemannian geometry for three datasets. The orange surfaces represent the manifolds learned by the model, while the blue points correspond to the training data. Each manifold provides a convincing low-dimensional representation of the data, isometric to its respective latent space.
    }
    \label{fig:learned_charts}
\end{figure*}

% e.g., from the standard $\ell^2$-inner product reweighed by the inverse of the local density \cite{sorrenson2024learningdistancesdatanormalizing}.
% or by assuming a locally adaptive normal distribution \cite{arvanitidis2016locally}.


% Subsequently, diffusion models can come into play through constructing density-based Riemannian geometry, e.g., from the standard $\ell^2$-inner product reweighed by the inverse of the local density, which has been demonstrated to yield geodesics through the data density in practice \cite{sorrenson2024learningdistancesdatanormalizing}.

If the manifold mapping scalability challenges were to be overcome, the combined power of Riemannian geometry and state of the art generative modelling could have profound implications on how to handle data in general. 
Indeed, beyond typical data analysis tasks such as computing distances, means, and interpolations/extrapolations of data points,
% as illustrated in \Cref{fig:toy-example-barycentre,fig:toy-example-geodesic,fig:toy-example-log,fig:toy-example-exp}
a data-driven Riemannian structure also offers greater potential for representation learning and downstream applications. For instance, many advanced data processing methods, from Principal Component Analysis (PCA) to score and flow-matching, have Riemannian counterparts (\citet{diepeveen2023curvature,fletcher2004principal} and \citet{chen2023riemannian,huang2022riemannian}) that have proven beneficial by improving upon full black box methods in terms of interpretability \citep{diepeveen2024pulling} or Euclidean counterparts in terms of efficiency \citep{kapusniak2024metricflowmatchingsmooth,de2024pullback}. 
% For example, applications of these methods have recently shown promising results in interpretable representation learning \citep{diepeveen2024pulling}
% \footnote{where the latent space can be constructed to be isometric with the data manifold, which is a feature standard Variational Autoencoders (VAE) \cite{kingma2013auto} do not have.}
% and in downstream tasks such as data generation . 
Here it is worth highlighting that scalability of manifold mappings was completely circumvented by \cite{diepeveen2024pulling} and \cite{de2024pullback} by using pullback geometry. 
However, here learning a suitable (and stable) pullback geometry suffers from challenges regarding \emph{scalability of the training algorithm}, contrary to the approach by \cite{sorrenson2024learningdistancesdatanormalizing}.

% However, these methods typically require cheap access to manifold mappings such as geodesics, logarithmic and exponential mappings or even symmetry of the Riemannian structure, which is in general not the case in the density-based approaches by \cite{sorrenson2024learningdistancesdatanormalizing} or LAND \cite{arvanitidis2016locally}, but comes for free if the Riemannian structure were to come in pullback form \cite{diepeveen2024pulling}.

% Moreover, these Riemannian approaches provide enhanced interpretability, particularly in relation to Variational Autoencoders (VAEs).

% \cite{arvanitidis2016locally} % locally adaptive diagonal metric tensor constructed from a data set
 % \cite{hauberg2012geometric} % metric learning with gaussian interpretation
 % \cite{peltonen2004improved} % fisher information on conditional density, but do not actually try to compute geodesics
 % \cite{Scarvelis2023} 

% Motivated by the above, in this work we are concerned with the following question: if we have access to the data probability density or related weaker notions such as its score obtained from a diffusion model \cite{song2020score}, when and how can we construct a Riemannian structure that has computationally feasible manifold mappings?

Motivated by the above, this work aims to address the following question: How to strike a good balance between scalability of training a data-driven Riemannian structure and of evaluating its corresponding manifold mappings?

% Given access to the data probability density, or related weaker notions such as the score, when and how can we construct a Riemannian structure that allows for computationally feasible manifold mappings as illustrated in \Cref{fig:toy-example-barycentre,fig:toy-example-geodesic,fig:toy-example-log,fig:toy-example-exp} and how do we find such structures from data? 

% \todo{ZS: I think this sentence is unnecessary} In particular, in this work we consider how we can combine best practices from density-based Riemannian geometry \cite{sorrenson2024learningdistancesdatanormalizing} and data-driven pullback-based Riemannian geometry \cite{diepeveen2024pulling}.

% [end with problem of trying to get Riemannian geometry from the score]

% \begin{figure}[h!]
%     \centering
%     % \begin{subfigure}{0.19\linewidth}
%     %     \includegraphics[width=\linewidth]{../results/banana-distribution/rae_manifold.eps}
%     %     \caption{{Manifold (RAE)}}
%     %     \label{fig:toy-example-manifold}
%     % \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{results/banana-distribution/barycentre.png}
%         \caption{{Barycentre}}
%         \label{fig:toy-example-barycentre}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{results/banana-distribution/geodesic.png}
%         \caption{{Geodesic}}
%         \label{fig:toy-example-geodesic}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{results/banana-distribution/logarithmic.png}
%         \caption{{Logarithm}}
%         \label{fig:toy-example-log}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=\linewidth]{results/banana-distribution/exponential.png}
%         \caption{{Exponential}}
%         \label{fig:toy-example-exp}%
%     \end{subfigure}
%     \caption{
%     % Score-based pullback Riemannian geometry 
%     Proposed Riemannian geometry from a toy probability density, visualized by its level sets.}
%     \label{fig:toy-example}
% \end{figure}
% \todo{fix captions}
% \todo{say in the figure caption that these are toy examples, but are also the result of our work.}

% \subsection{Related work}

% [short sentence here saying that both density-based approaches and pullback approaches have their ups and downs.]

% \paragraph{Density-based Riemannian geometry}
% % [here we mean we try to learn the actual density and use that to construct RG]
% % This line of research can be traced back at least to early works such as
% % % [Little, Sorrrenson]
% % \cite{bousquet2003measure}
% % \cite{sajama2005estimating}
% % where the idea of using the data density to define and compute geodesics was proposed. [It should be highlighted that these approaches used a discrete data set from which the density and the geodesics were estimated, but not the density itself, which would yield an actual Riemannian structure across all of space.]
% % This approach was continued by 
% % \cite{bijral2012semi}, which was soon followed by a line of theoretical contributions on convergence of power-weighted shortest path distances to geodesic distances under the density-dependent Riemannian metric  
% % \cite{alamgir2012shortest,chu2020exact,groisman2022nonhomogeneous,hwang2012shortest,little2020path,little2022balancing,mckenzie2019power,moscovich2017minimax}. Only recently, the leap to estimating the full density and using it to construct Riemannian geometry on all of space was made by \cite{sorrenson2024learningdistancesdatanormalizing} who use the scalability of normalizing flows and diffusion models and their training schemes. However, as mentioned above, even though the density can be obtained in a scalable way, the manifold mappings are still computationally expensive despite several smart relaxations in the geodesic equation that is solved.

% This line of research dates back to early works such as \cite{bousquet2003measure} and \cite{sajama2005estimating}, where the idea of using data density to define and compute geodesics was first proposed. It is important to note that these approaches relied on discrete data sets to estimate density and geodesics on and through the data points, rather than utilizing a parametrization of the density itself to create a Riemannian structure across the entire space. This approach was further developed by \cite{bijral2012semi}, leading to a series of theoretical contributions on the convergence of power-weighted shortest path distances to geodesic distances under a density-dependent Riemannian metric \cite{alamgir2012shortest,chu2020exact,groisman2022nonhomogeneous,hwang2012shortest,little2020path,little2022balancing,mckenzie2019power,moscovich2017minimax}. \todo{ZS: What about limitations of these?}

% Most of the works above however rely primarily on sampled data for extracting intrinsic geometry. This often comes with an impossible cost of scaling in terms of data \todo{ZS: Willem, what else could fall into limitations?}. 

% Recently, \citet{sorrenson2024learningdistancesdatanormalizing} proposed learning the probability density and using it directly to construct Riemannian geometry across the entire space, leveraging the scalability of normalizing flows and diffusion models along with their training schemes. However, despite this, obtaining manifold mappings remains computationally expensive, even with several clever relaxations in solving the geodesic equation. 

% As a result, two important questions still remain unanswered: given a distribution, what should the intrinsic geometry be and how can manifold mappings for this geometry be made computationally feasible? 

% % \cite{hauberg2012geometric} % more metric learning between classes

% % [2, 42, 62]
%  % ?
 
% \paragraph{Pullback-based Riemannian geometry}
% % [construct diffeomorphisms and Pullback geometry ]
% % The pullback framework, in which a diffeomorphism is learned for a data driven Riemannian structure, has the opposite problem. That is works such as
% %  \cite{cuzzolin2008learning}
% %  \cite{gruffaz2021learning}
% %  % \cite{hauser2017principles}
% %  \cite{Lebanon2006}
% %  have closed-form manifold mappings, but their respective learning problems assumes a specific problem to be solved unrelated to estimating the data density, which is not general. The only general setting is by \cite{diepeveen2024pulling} shows promising results, but the learning problem does not scale well with the amount of data, which can potentially be problematic in terms of scalability.

% The pullback framework, which involves learning a diffeomorphism for a data-driven Riemannian structure, come with closed-form manifold mappings, but come with different challenges. In works such as \cite{cuzzolin2008learning,gruffaz2021learning,Lebanon2006} their learning problems are tailored to specific tasks unrelated to estimating data density, thus lacking generality. \cite{diepeveen2024pulling} presents a more general approach, which shows promising results, but has the opposite problem to the density-based approach by \cite{sorrenson2024learningdistancesdatanormalizing}. That is, here the learning problem suffers from scalability issues with increasing data size.



% % [data-driven Riemannian geometry]

% % [end with dichotomy between pullback work and density based-RG and perhaps pros and cons (closed-form mappings on the one hand and scalability on the other)]

% % In particular, how can we combine best practices from data-driven pullback-based Riemannian geometry \cite{diepeveen2024pulling} and density-based Riemannian geometry \cite{sorrenson2024learningdistancesdatanormalizing}?

\subsection{Contributions}
% Motivated by the above, we aim to bridge this gap between only having scalability of the learning problem as in density-based Riemannian geometry and only having scalability of the manifold mappings as in pullback-based Riemannian geometry. In particular, in this work we consider a family of unimodal probability densities, whose negative log likelihoods are compositions of strongly convex functions and diffeomorphisms. 
% \begin{itemize}
%     \item We propose a density-based  Riemannian structure that comes in pullback form, and in the case where the strongly convex function is Gaussian, boils down to the Riemannian structure from \cite{diepeveen2024pulling} which allows to use their theory
%     \item We show that such a density-based Riemannian structure naturally generates a Riemannian Autoencoder with error bounds on the expected reconstruction error
%     \item We propose a learning scheme based on [normalizing flow/diffusion model] learning to find the distribution that is to be plugged into the Riemannian framework
% \end{itemize}


In this paper, we take first steps towards striking such a balance and propose a score-based pullback Riemannian metric assuming a relatively simple but generally applicable family of probability densities, which we show to result in both scalable manifold mappings and scalable learning algorithms. We emphasize that we do not directly aim to find the perfect balance between the two types of scalability. Instead we start from a setting which has many nice properties, but will allow for generalization to multimodal densities, which we reserve for future work.
% Inspired by the above, our goal is to bridge the gap between the scalability of learning problems in density-based Riemannian geometry, which lacks scalable manifold mappings, and the scalability of manifold mappings in pullback-based Riemannian geometry, which lacks scalable learning problems. 


% \todo{Technically no longer unimodal?}
Specifically, we consider a family of unimodal probability densities whose negative log-likelihoods are compositions of strongly convex functions and diffeomorphisms. As this work is an attempt to bridge between the geometric data analysis community and the generative modeling community, we break down the contributions in two ways.
Theoretically,
\begin{itemize}
    % \item \new 
    % We show that in analogy with the fisher information metric, considering the symmetrized KL divergence between denoising posteriors naturally results in a pullback - based metric.
    \item We propose a score-based pullback Riemannian metric such that manifold mappings respect the data distribution.
    % as illustrated in \Cref{fig:toy-example-barycentre,fig:toy-example-geodesic,fig:toy-example-log,fig:toy-example-exp}.
    \item We demonstrate that this density-based Riemannian structure naturally leads to a Riemannian autoencoder\footnote{in the sense of \citet{diepeveen2024pulling}} and provide error bounds on the expected reconstruction error, which allows for approximation of the data manifold as illustrated in \Cref{fig:learned_charts}.
    \item We introduce a learning scheme based on adaptations of normalizing flows to find the density to be integrated into the Riemannian framework, which is tested on several synthetic data sets. 
\end{itemize}
Practically, this work showcases how two simple adaptations to the normalizing flows framework enable data-driven Riemannian geometry. This significantly expands the potential for downstream applications compared to the unadapted framework.


% \todo{ZS: The current version seems to overcite Willems work I think?}

% [consider unimodal case, which gives closed-form manifold mappings, and gaussian case which links nicely to prior work, from which we can use theory]

% [RAE with guarantees]

% [Training scheme]

\subsection{Outline}

After introducing notation in \Cref{sec:notation}, \Cref{sec:unimodal-riemannian geometry} considers a family of probability distributions, from which we obtain suitable geometry, and \Cref{sec:rae} showcases how one can subsequently construct Riemannian Autoencoders with theoretical guarantees. From these observations \Cref{sec:adapting-normalizing-flows} discusses the natural limitations of standard normalizing flows and how to change the parametrisation and training for downstream application in a Riemannian geometric setting. \Cref{sec:numerics} showcases several use cases of data-driven Riemannian structure on several data sets. Finally, we summarize our findings in \Cref{sec:conclusions}.


==> sections/1-introduction.tex <==
\section{Introduction (2 pages)}

% Data tend to live near low dimensional non-linear  manifolds as in \cref{fig:toy-example-manifold}. This manifold assumption \cite{fefferman2016testing} has been popular ever since early work on non-linear dimension reduction \cite{belkin2001laplacian,coifman2006diffusion,roweis2000nonlinear,sammon1969nonlinear,tenenbaum2000global} and can still be observed from more modern machine learning approaches such as diffusion models \cite{song2020score} in recent works such as \cite{sakamoto2024the,stanczuk2022your}. Actually learning this non-linear structure, or learning a representation, from data has been very successful \cite{demers1992non,kingma2013auto} and remains an active area of research.

Data often reside near low-dimensional non-linear manifolds as illustrated in \cref{fig:toy-example-manifold}. This manifold assumption \cite{fefferman2016testing} has been popular since the early work on non-linear dimension reduction \cite{belkin2001laplacian,coifman2006diffusion,roweis2000nonlinear,sammon1969nonlinear,tenenbaum2000global}. Learning this non-linear structure, or representation learning, from data has proven to be highly successful \cite{demers1992non,kingma2013auto} and continues to be relevant\todo{ZS: What do you mean relevant?} in modern machine learning approaches, with researchers noting that diffusion models \cite{song2020score} often identify the manifold, as evidenced in recent studies \cite{sakamoto2024the,stanczuk2022your}. 
% Learning this non-linear structure, or representation learning, from data has proven to be highly successful \cite{demers1992non,kingma2013auto} and remains an active area of research.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{../results/banana-distribution/distribution.eps}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% In particular, data-driven Riemannian geometry has recently shown to be a suitable language to learn representations. In this setting, representations are elements living in a geodesic subspace  \cite{arvanitidis2016locally,diepeveen2024pulling,hauberg2012geometric,peltonen2004improved,Scarvelis2023,sorrenson2024learningdistancesdatanormalizing} of the data space under a non-trivial Riemannian structure, i.e., other than the $\ell^2$-inner product on all of space. 
% Besides standard data analysis tasks such as computing distances, means, interpolates and extrapolates of data points, a data-driven Riemannian structure has more potential for representation learning and for downstream problems. For example, many more advanced data processing methods from PCA \cite{fletcher2004principal,diepeveen2023curvature} to flow-matching \cite{chen2023riemannian} have Riemannian counterparts, which have shown fruitful in applications in representation learning with the recent introduction of the curvature corrected Riemannian autoencoder\footnote{Note On top of that gives more interpretatbility [e.g., wrt VAE]]} (CC-RAE) \cite{diepeveen2024pulling} and in downstream tasks such as generation \cite{kapusniak2024metricflowmatchingsmooth}.

Recent advances in data-driven Riemannian geometry have demonstrated its suitability for learning representations and possible combinations with findings from the diffusion model literature. \todo{ZS: I dont understand this sentence} In this context, representations are elements residing in a geodesic subspace of the data space, governed by a non-trivial Riemannian structure, rather than the standard $\ell^2$-inner product across the entire space \cite{arvanitidis2016locally,diepeveen2024pulling,hauberg2012geometric,peltonen2004improved,Scarvelis2023,sorrenson2024learningdistancesdatanormalizing}. 
\new Subsequently, information about the data distribution, in the form of the density or the score can be used to construct a Riemannian structure e.g., from the standard $\ell^2$-inner product reweighed by the inverse of the local density \cite{sorrenson2024learningdistancesdatanormalizing} or by assuming a locally adaptive normal distribution \cite{arvanitidis2016locally}.


% Subsequently, diffusion models can come into play through constructing density-based Riemannian geometry, e.g., from the standard $\ell^2$-inner product reweighed by the inverse of the local density, which has been demonstrated to yield geodesics through the data density in practice \cite{sorrenson2024learningdistancesdatanormalizing}.

Beyond typical data analysis tasks such as computing distances, means, and interpolations/extrapolations of data points, a data-driven Riemannian structure also offers greater potential for representation learning and downstream applications. For instance, many advanced data processing methods, from Principal Component Analysis (PCA) to score and flow-matching, have Riemannian counterparts \cite{fletcher2004principal,diepeveen2023curvature} and \cite{chen2023riemannian,huang2022riemannian} that have proven beneficial. 
\new However, the literature so far has primarily concerned itself with developing methods that are able to utilize extrinsic information about the geometry of the problem. In this paper, on the other hand, we consider the problem of extracting the intrinsic geometric information out of data.

Methods utilizing intrinsic geometry have recently shown promise in interpretable representation learning, particularly with the introduction of the Riemannian Autoencoder (RAE) \cite{diepeveen2024pulling}\footnote{where the latent space can be constructed to be isometric with the data manifold, which is a feature standard Variational Autoencoders (VAE) \cite{kingma2013auto} do not have.}, and in downstream tasks such as data generation \cite{kapusniak2024metricflowmatchingsmooth}. However, these methods typically require cheap access to manifold mappings such as geodesics, logarithmic and exponential mappings or even symmetry of the Riemannian structure, which is in general not the case in the density-based approaches by \cite{sorrenson2024learningdistancesdatanormalizing} or LAND \cite{arvanitidis2016locally}, but comes for free if the Riemannian structure were to come in pullback form \cite{diepeveen2024pulling}.

% Moreover, these Riemannian approaches provide enhanced interpretability, particularly in relation to Variational Autoencoders (VAEs).

% \cite{arvanitidis2016locally} % locally adaptive diagonal metric tensor constructed from a data set
 % \cite{hauberg2012geometric} % metric learning with gaussian interpretation
 % \cite{peltonen2004improved} % fisher information on conditional density, but do not actually try to compute geodesics
 % \cite{Scarvelis2023} 

% Motivated by the above, in this work we are concerned with the following question: if we have access to the data probability density or related weaker notions such as its score obtained from a diffusion model \cite{song2020score}, when and how can we construct a Riemannian structure that has computationally feasible manifold mappings?

Motivated by the above, this work aims to addresses the following question: Given access to the data probability density, or related weaker notions such as the score, when and how can we construct a Riemannian structure that allows for computationally feasible manifold mappings as illustrated in \cref{fig:toy-example-barycentre,fig:toy-example-geodesic,fig:toy-example-log,fig:toy-example-exp} and how do we find such structures from data? 

\todo{ZS: I think this sentence is unnecessary} In particular, in this work we consider how we can combine best practices from density-based Riemannian geometry \cite{sorrenson2024learningdistancesdatanormalizing} and data-driven pullback-based Riemannian geometry \cite{diepeveen2024pulling}.

% [end with problem of trying to get Riemannian geometry from the score]

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.19\linewidth}
        \includegraphics[width=\linewidth]{../results/banana-distribution/rae_manifold.eps}
        \caption{}
        \label{fig:toy-example-manifold}
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}
        \includegraphics[width=\linewidth]{../results/banana-distribution/barycentre.eps}
        \caption{}
        \label{fig:toy-example-barycentre}
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}
        \includegraphics[width=\linewidth]{../results/banana-distribution/geodesic.eps}
        \caption{}
        \label{fig:toy-example-geodesic}
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}
        \includegraphics[width=\linewidth]{../results/banana-distribution/logarithmic.eps}
        \caption{}
        \label{fig:toy-example-log}
    \end{subfigure}
    \begin{subfigure}{0.19\linewidth}
        \includegraphics[width=\linewidth]{../results/banana-distribution/exponential.eps}
        \caption{}
        \label{fig:toy-example-exp}
    \end{subfigure}
    \caption{Caption. TODO}
    \label{fig:toy-example}
\end{figure}
\todo{say in the figure caption that these are toy examples, but are also the result of our work.}

\subsection{Related work}

[short sentence here saying that both density-based approaches and pullback approaches have their ups and downs.]

\paragraph{Density-based Riemannian geometry}
% [here we mean we try to learn the actual density and use that to construct RG]
% This line of research can be traced back at least to early works such as
% % [Little, Sorrrenson]
% \cite{bousquet2003measure}
% \cite{sajama2005estimating}
% where the idea of using the data density to define and compute geodesics was proposed. [It should be highlighted that these approaches used a discrete data set from which the density and the geodesics were estimated, but not the density itself, which would yield an actual Riemannian structure across all of space.]
% This approach was continued by 
% \cite{bijral2012semi}, which was soon followed by a line of theoretical contributions on convergence of power-weighted shortest path distances to geodesic distances under the density-dependent Riemannian metric  
% \cite{alamgir2012shortest,chu2020exact,groisman2022nonhomogeneous,hwang2012shortest,little2020path,little2022balancing,mckenzie2019power,moscovich2017minimax}. Only recently, the leap to estimating the full density and using it to construct Riemannian geometry on all of space was made by \cite{sorrenson2024learningdistancesdatanormalizing} who use the scalability of normalizing flows and diffusion models and their training schemes. However, as mentioned above, even though the density can be obtained in a scalable way, the manifold mappings are still computationally expensive despite several smart relaxations in the geodesic equation that is solved.

This line of research dates back to early works such as \cite{bousquet2003measure} and \cite{sajama2005estimating}, where the idea of using data density to define and compute geodesics was first proposed. It is important to note that these approaches relied on discrete data sets to estimate density and geodesics on and through the data points, rather than utilizing a parametrization of the density itself to create a Riemannian structure across the entire space. This approach was further developed by \cite{bijral2012semi}, leading to a series of theoretical contributions on the convergence of power-weighted shortest path distances to geodesic distances under a density-dependent Riemannian metric \cite{alamgir2012shortest,chu2020exact,groisman2022nonhomogeneous,hwang2012shortest,little2020path,little2022balancing,mckenzie2019power,moscovich2017minimax}. \todo{ZS: What about limitations of these?}

Most of the works above however rely primarily on sampled data for extracting intrinsic geometry. This often comes with an impossible cost of scaling in terms of data \todo{ZS: Willem, what else could fall into limitations?}. 

Recently, \citet{sorrenson2024learningdistancesdatanormalizing} proposed learning the probability density and using it directly to construct Riemannian geometry across the entire space, leveraging the scalability of normalizing flows and diffusion models along with their training schemes. However, despite this, obtaining manifold mappings remains computationally expensive, even with several clever relaxations in solving the geodesic equation. 

As a result, two important questions still remain unanswered: given a distribution, what should the intrinsic geometry be and how can manifold mappings for this geometry be made computationally feasible? 

% \cite{hauberg2012geometric} % more metric learning between classes

% [2, 42, 62]
 % ?
 
\paragraph{Pullback-based Riemannian geometry}
% [construct diffeomorphisms and Pullback geometry ]
% The pullback framework, in which a diffeomorphism is learned for a data driven Riemannian structure, has the opposite problem. That is works such as
%  \cite{cuzzolin2008learning}
%  \cite{gruffaz2021learning}
%  % \cite{hauser2017principles}
%  \cite{Lebanon2006}
%  have closed-form manifold mappings, but their respective learning problems assumes a specific problem to be solved unrelated to estimating the data density, which is not general. The only general setting is by \cite{diepeveen2024pulling} shows promising results, but the learning problem does not scale well with the amount of data, which can potentially be problematic in terms of scalability.

The pullback framework, which involves learning a diffeomorphism for a data-driven Riemannian structure, come with closed-form manifold mappings, but come with different challenges. In works such as \cite{cuzzolin2008learning,gruffaz2021learning,Lebanon2006} their learning problems are tailored to specific tasks unrelated to estimating data density, thus lacking generality. \cite{diepeveen2024pulling} presents a more general approach, which shows promising results, but has the opposite problem to the density-based approach by \cite{sorrenson2024learningdistancesdatanormalizing}. That is, here the learning problem suffers from scalability issues with increasing data size.



% [data-driven Riemannian geometry]

% [end with dichotomy between pullback work and density based-RG and perhaps pros and cons (closed-form mappings on the one hand and scalability on the other)]

% In particular, how can we combine best practices from data-driven pullback-based Riemannian geometry \cite{diepeveen2024pulling} and density-based Riemannian geometry \cite{sorrenson2024learningdistancesdatanormalizing}?

\subsection{Contributions}
% Motivated by the above, we aim to bridge this gap between only having scalability of the learning problem as in density-based Riemannian geometry and only having scalability of the manifold mappings as in pullback-based Riemannian geometry. In particular, in this work we consider a family of unimodal probability densities, whose negative log likelihoods are compositions of strongly convex functions and diffeomorphisms. 
% \begin{itemize}
%     \item We propose a density-based  Riemannian structure that comes in pullback form, and in the case where the strongly convex function is Gaussian, boils down to the Riemannian structure from \cite{diepeveen2024pulling} which allows to use their theory
%     \item We show that such a density-based Riemannian structure naturally generates a Riemannian Autoencoder with error bounds on the expected reconstruction error
%     \item We propose a learning scheme based on [normalizing flow/diffusion model] learning to find the distribution that is to be plugged into the Riemannian framework
% \end{itemize}

Given the recent rise in interest in generative models, a natural question arises: can we use the learned density/score to extract the intrinsic geometry of the data? 

In this paper, we propose a score-based (pullback) Riemannian metric, which we show to result in both scalable manifold mappings (unlike density-based Riemannian geometries) AND scalable learning algorithms (unlike pullback-based Riemannian geometry).
% Inspired by the above, our goal is to bridge the gap between the scalability of learning problems in density-based Riemannian geometry, which lacks scalable manifold mappings, and the scalability of manifold mappings in pullback-based Riemannian geometry, which lacks scalable learning problems. 


\todo{Technically no longer unimodal?}
Specifically, we consider a family of unimodal probability densities whose negative log-likelihoods are compositions of strongly convex functions and diffeomorphisms.
Theoretically,
\begin{itemize}
    \item \new 
    We show that in analogy with the fisher information metric, considering the symmetrized KL divergence between denoising posteriors naturally results in a pullback - based metric.
    \item We propose a density-based Riemannian structure in pullback form, reducing to the structure from \cite{diepeveen2024pulling} when using a quadratic function, thus leveraging their theory.
    \item We demonstrate that this density-based Riemannian structure naturally leads to a Riemannian Autoencoder, providing error bounds on the expected reconstruction error.
    \item We introduce a learning scheme based on [normalizing flows or diffusion models]\todo{pick one or leave both} to find the density to be integrated into the Riemannian framework, which is tested on several synthetic data sets. 
\end{itemize}
Practically,

\todo{ZS: The current version seems to overcite Willems work I think?}

% [consider unimodal case, which gives closed-form manifold mappings, and gaussian case which links nicely to prior work, from which we can use theory]

% [RAE with guarantees]

% [Training scheme]

\subsection{Outline}

\todo[inline]{TODO}

==> sections/2-notation.tex <==
\section{Notation}
\label{sec:notation}

% \subsection{Differential Geometry}
Here we present some basic notations from differential and Riemannian geometry, see \citet{boothby2003introduction,carmo1992riemannian,lee2013smooth,sakai1996riemannian} for details. 
% \dn{What does this sentence mean exactly? Maybe instead say something like "Here we present some basics and notation from differential and Riemannian geometry, see \cite{}... for more details." ?} \wdp{fixed}


Let $\manifold$ be a smooth manifold. We write $C^\infty(\manifold)$ for the space of smooth functions over $\manifold$. The \emph{tangent space} at $\mPoint \in \manifold$, which is defined as the space of all \emph{derivations} at $\mPoint$, is denoted by $\tangent_\mPoint \manifold$ and for \emph{tangent vectors} we write $\tangentVector_\mPoint \in \tangent_\mPoint \manifold$. For the \emph{tangent bundle} we write $\tangent\manifold$ and smooth vector fields, which are defined as \emph{smooth sections} of the tangent bundle, are written as $\vectorfield(\manifold) \subset \tangent\manifold$.
% Furthermore, additional structure on manifolds and derived notions thereof are typically defined through tensor fields of the form $T~:~\vectorfield(\manifold)^n \to \vectorfield(\manifold)^m$ or $T~:~\vectorfield(\manifold)^n \to C^\infty(\manifold)$. A tensor field can -- by definition of being $C^\infty(\manifold)$-modules -- be restricted to a tangent space at each point $\mPoint \in \manifold$, for which we use the notation $T_{\mPoint}: \tangent_\mPoint \manifold^n \to \tangent_\mPoint \manifold^m$ or $T_{\mPoint}: \tangent_\mPoint \manifold^n \to \Real$. 

A smooth manifold $\manifold$ becomes a \emph{Riemannian manifold} if it is equipped with a smoothly varying \emph{metric tensor field} $(\,\cdot\,, \,\cdot\,) \colon \vectorfield(\manifold) \times \vectorfield(\manifold) \to C^\infty(\manifold)$. This tensor field induces a \emph{(Riemannian) metric} $\distance_{\manifold} \colon \manifold\times\manifold\to\Real$. The metric tensor can also be used to construct a unique affine connection, the \emph{Levi-Civita connection}, that is denoted by $\nabla_{(\,\cdot\,)}(\,\cdot\,) : \vectorfield(\manifold) \times \vectorfield(\manifold) \to \vectorfield(\manifold)$. 
This connection is in turn the cornerstone of a myriad of manifold mappings.
One is the notion of a \emph{geodesic}, which for two points $\mPoint,\mPointB \in \manifold$ is defined as a curve $\geodesic_{\mPoint,\mPointB} \colon [0,1] \to \manifold$ with minimal length that connects $\mPoint$ with $\mPointB$. 
Another closely related notion to geodesics is the curve $t \mapsto \geodesic_{\mPoint,\tangentVector_\mPoint}(t)$  for a geodesic starting from $\mPoint\in\manifold$ with velocity $\dot{\geodesic}_{\mPoint,\tangentVector_\mPoint} (0) = \tangentVector_\mPoint \in \tangent_\mPoint\manifold$. This can be used to define the \emph{exponential map} $\exp_\mPoint \colon \mathcal{D}_\mPoint \to \manifold$ as 
\begin{equation}
\exp_\mPoint(\tangentVector_\mPoint) := \geodesic_{\mPoint,\tangentVector_\mPoint}(1)
\quad\text{where $\mathcal{D}_\mPoint \subset \tangent_\mPoint\manifold$ is the set on which $\geodesic_{\mPoint,\tangentVector_\mPoint}(1)$ is defined.} 
\end{equation}
% The manifold $\manifold$ is said to be \emph{(geodesically) complete} whenever $\mathcal{D}_\mPoint = \mathcal{T}_{\mPoint}\manifold$ for all $\mPoint \in \manifold$.
Furthermore, the \emph{logarithmic map} $\log_\mPoint \colon \exp(\mathcal{D}'_\mPoint ) \to \mathcal{D}'_\mPoint$ is defined as the inverse of $\exp_\mPoint$, so it is well-defined on  $\mathcal{D}'_{\mPoint} \subset \mathcal{D}_{\mPoint}$ where $\exp_\mPoint$ is a diffeomorphism. 
% The connection can also be used to identify tangent vectors in different tangent spaces through the \emph{parallel transport mapping} $\mathcal{P}_{\mPointB \leftarrow \mPoint}: \mathcal{T}_{\mPoint}\manifold\to \mathcal{T}_{\mPointB}\manifold$. 

Finally, if $(\manifold, (\cdot,\cdot))$ is a $\dimInd$-dimensional Riemannian manifold, $\manifoldB$ is a $\dimInd$-dimensional smooth manifold and $\diffeoB:\manifoldB \to \manifold$ is a diffeomorphism, the \emph{pullback metric}
\begin{equation}
    (\tangentVector, \tangentVectorB)^\diffeoB := (D_{(\cdot)}\diffeoB[\tangentVector_{(\cdot)}], D_{(\cdot)}\diffeoB[\tangentVectorB_{(\cdot)}])_{\diffeoB(\cdot)},
    \label{eq:pull-back-metric}
\end{equation}
where $D_{\mPoint}\diffeoB: \tangent_\mPoint \manifoldB \to \tangent_{\diffeoB(\mPoint)} \manifold$ denotes the differential of $\diffeoB$,
% or 
% \begin{equation}
%     (\tangentVector, \tangentVectorB)^\diffeoB := (\diffeoB_*[\tangentVector], \diffeoB_*[\tangentVectorB])
%     \label{eq:pull-back-metric}
% \end{equation}
defines a Riemannian structure on $\manifoldB$, which we denote by $(\manifoldB, (\cdot,\cdot)^\diffeoB)$. 
Pullback metrics literally pull back all geometric information from the Riemannian structure on $\manifold$. In particular, closed-form manifold mappings on $(\manifold, (\cdot,\cdot))$ yield under mild assumptions closed-form manifold mappings on $(\manifoldB, (\cdot,\cdot)^\diffeoB)$.
Throughout the rest of the paper pullback mappings will be denoted similarly to \cref{eq:pull-back-metric} with the diffeomorphism $\diffeoB$ as a superscript, i.e., we write $\distance^\diffeoB_{\manifoldB}(\mPoint, \mPointB)$, $\geodesic^\diffeoB_{\mPoint, \mPointB}$, $\exp^\diffeoB_\mPoint (\tangentVector_\mPoint)$ and $\log^\diffeoB_{\mPoint} \mPointB$ 
% and $\mathcal{P}^\diffeoB_{\mPointB \leftarrow \mPoint} \tangentVector_\mPoint$ 
for $\mPoint,\mPointB \in \manifoldB$ and $\tangentVector_\mPoint \in \tangent_\mPoint \manifoldB$. 

% In \Cref{app:proofs-prelim-pullback-geometry-theoretical-results} we state several \emph{known results} for Riemannian geometry on $(\Real^\dimInd, (\cdot,\cdot)^\diffeoB)$, where the mapping $\diffeoB:\Real^\dimInd \to \manifold$ is a diffeomorphism and $(\manifold, (\cdot,\cdot))$ is a $\dimInd$-dimensional Riemannian manifold. In particular, we will remind the reader that we can pull back basic mappings and additional structure, e.g., symmetry. For the sake of completeness, the proofs are also provided in \Cref{app:proofs-prelim-pullback-geometry-theoretical-results}. Regarding notation, throughout the rest of the paper pullback mappings will be denoted similarly to \cref{eq:pull-back-metric} with the diffeomorphism $\diffeoB$ as a superscript, i.e., we write $\distance^\diffeoB_{\Real^\dimInd}(\mPoint, \mPointB)$, $\geodesic^\diffeoB_{\mPoint, \mPointB}$, $\exp^\diffeoB_\mPoint (\tangentVector_\mPoint)$, $\log^\diffeoB_{\mPoint} \mPointB$ and $\mathcal{P}^\diffeoB_{\mPointB \leftarrow \mPoint} \tangentVector_\mPoint$ for $\mPoint,\mPointB \in \Real^\dimInd$ and $\tangentVector_\mPoint \in \tangent_\mPoint \Real^\dimInd$. 


% \subsection{Normalizing Flows}
% \todo{WD: we are not using this notation. Why mention it?}
% \todo{ZS: Oh we can adapt the notation to match the rest of the paper - this was just for the sake of introducing normalzing flows}
% \todo{WD: we only use it once and adapt it immediately. So I think there will be no confusion if we skip it here. We would also have more space for experiments.}
% The normalizing flow \cite{dinh2017density} is an approach to density estimation defined through a parameterized invertible mapping $\diffeoB: \mathcal{X} \rightarrow \mathcal{Z}$ from the data space $\mathcal{X}$ to a latent space $\mathcal{Z}$. The data distribution is modelled as a transformation $\diffeoB^{-1}: \mathcal{Z} \rightarrow \mathcal{X}$ applied to a random variable from the latent distribution $z \sim p_{\mathcal{Z}}$, often chosen to be Gaussian. The density of the transformed random variable $x=\diffeoB^{-1}(z)$ is given by the change of variables formula
% \begin{equation}\label{eq:nf}
% p_{\mathcal{X}}(\Vector)=p_{\mathcal{Z}}(\diffeoB(\Vector)) \cdot\left|\operatorname{det}\left(D_{\Vector} \diffeoB\right)\right|    
% \end{equation}
% The mapping $\diffeoB$ is implemented as a sequence of invertible transformations, parametrized by a neural network with parameters $\Theta$ and an architecture ensuring invertibility and efficient computation of log-determinants. The model is trained by maximizing the likelihood in \cref{eq:nf} of the training data with respect to the parameters $\Theta$.

% % But here is the thing - if $J_{\diffeoB}(x)$ (or $D_{\Vector}\diffeoB$) is an orthogonal operator, then what we have is that $\score(x) = \left[\nabla \log p_u\right](\diffeoB(x))$, so if $\log p_u$ is strongly convex, then the normalizing flow score is equivalent to the pseudo-score below.

==> sections/3-data-analysis-nf-oriented.tex <==
\section{Riemannian geometry from unimodal probability densities}
\label{sec:unimodal-riemannian geometry}

% \todo{I propose to first define the metric in its most general form from the score, then followed by this section - want to keep this as general as we can for as long as we can.}
We remind the reader that the ultimate goal of data-driven Riemannian geometry on $\Real^\dimInd$ is to construct a Riemannian structure such that geodesics always pass through the support of data probability densities. In this section we will focus on constructing Riemannian geometry that does just that from unimodal densities $\density:\Real^\dimInd\to \Real$ of the form
\begin{equation}
    \density(\Vector) \propto e^{- \stroco(\diffeo(\Vector))}
    \label{eq:stroco-diffeo-density}
\end{equation}
where $\stroco:\Real^\dimInd\to\Real$ is a smooth strongly convex function and $\diffeo:\Real^\dimInd\to\Real^\dimInd$ is a diffeomorphism, e.g., such as the density in \Cref{fig:toy-example}\footnote{Here, $\stroco(\Vector) := 2 \Vector_1^2 + \frac{1}{8}\Vector_2^2$ and $\diffeo(\Vector):= (\Vector_1 - \frac{1}{9} \Vector_2^2, \Vector_2)$.}. In particular, we will consider pullback Riemannian structures of the form
\begin{equation}
    (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector} := (D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB])_2,
    \label{eq:stroco-diffeo-pullback}
\end{equation}
which are related to the Riemannian structure obtained from the \emph{score function} $\nabla \log(\density(\cdot)):\Real^\dimInd\to\Real^\dimInd$ if $\diffeo$ is close to a linear $\ell^2$-isometry on the data support, i.e., $D_{\Vector} \diffeo$ is an orthogonal operator:
\begin{multline}
    (D_{\Vector} \nabla \log(\density(\cdot))[\tangentVector], D_{\Vector} \nabla \log(\density(\cdot))[\tangentVectorB])_2 = (D_{\Vector} \nabla (\stroco \circ \diffeo)[\tangentVector], D_{\Vector} \nabla (\stroco \circ \diffeo)[\tangentVectorB])_2 \\
    = (D_{\Vector} ((D_{(\cdot)} \diffeo)^{\top} \circ \nabla\stroco \circ \diffeo)[\tangentVector], D_{\Vector}((D_{(\cdot)} \diffeo)^{\top} \circ \nabla\stroco \circ \diffeo) [\tangentVectorB])_2 \\
    \approx (D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB])_2 = (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector}.
\end{multline}
For that reason, we call such an approach to data-driven Riemannian geometry: \emph{score-based pullback Riemannian geometry}. Since we find ourselves in a pullback setting\footnote{This is generally not true when using the score itself for probability densities of the form \cref{eq:stroco-diffeo-density}.}, this allows to construct pullback geometry with closed-form manifold mappings.

% \todo[inline]{Repeat that first of all this structure does what we want it to do as showcased in section 3.1.}

What remains to be shown is that such geodesics and other manifold mappings pass through the data support (like in \Cref{fig:toy-example-barycentre,fig:toy-example-geodesic,fig:toy-example-log,fig:toy-example-exp}). 
% \subsection{Manifold mappings}
% \label{sec:manifold-mappings}
The following result, which is a direct application of \citep[Prop.~2.1]{diepeveen2024pulling} and \citep[Cor.~3.6.1]{diepeveen2024pulling}, gives us closed-form expressions of several important manifold mappings under $(\cdot,\cdot)^{\nabla \stroco \circ \diffeo}$ and makes a connection with $(\cdot,\cdot)^{\diffeo}$ if we choose
\begin{equation}
    \stroco(\Vector)=\frac{1}{2} \Vector^{\top} \spdMatrix^{-1} \Vector,
    \label{eq:quadratic-stroco}
\end{equation}
where $\spdMatrix\in \Real^{\dimInd\times \dimInd}$ is symmetric positive definite. 

% This special case also makes it especially clear why we also in general get geodesics and manifold mappings that go through the data support. For example, in the case of \Cref{fig:toy-example}, which has the correct form \cref{eq:stroco-diffeo-density}, geodesics are just computed by undoing the effect of the diffeomporphism first -- so that the data distribution looks like a Gaussian -- and then computing straight lines between the data points. This will result in geodesics that move through regions with higher likelihoods than the end points, because of the strong convexity of the quadratic function, which is exactly what we want.

This special case highlights why, in general, we expect to obtain geodesics and manifold mappings that pass through the data support. For instance, in the scenario depicted in \Cref{fig:toy-example-geodesic}, where the correct form \cref{eq:stroco-diffeo-density} is used, geodesics are computed by first reversing the effect of the diffeomorphism -- transforming the data distribution to resemble a Gaussian, then drawing straight lines between the morphed data points, and finally applying the diffeomorphism again. This approach results in geodesics that traverse regions of higher likelihood between the endpoints, due to the strong convexity of the quadratic function, which aligns perfectly with our objectives. 

For the proof of the result below and a more general statement and proof related to geodesics passing through the data support as in explanation above, we refer the reader to \Cref{app:proof-of-basic-setup}.

\begin{proposition}
\label{thm:pull-back-mappings}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a smooth strongly convex function, whose Fenchel conjugate is denoted by $\stroco^\star: \Real^\dimInd\to\Real$. Next, consider the $\ell^2$-pullback manifolds $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ and $(\Real^\dimInd, (\cdot,\cdot)^{\diffeo})$ defined through metric tensor fields
    \begin{equation}
        (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector} := (D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB])_2, \quad \text{and} \quad (\tangentVector, \tangentVectorB)^{\diffeo}_{\Vector} := (D_{\Vector} \diffeo[\tangentVector], D_{\Vector} \diffeo[\tangentVectorB])_2.
    \end{equation}

    Then,
    \begin{enumerate}[label=(\roman*)]
        \item length-minimising geodesics $\geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}:[0,1] \to \Real^\dimInd$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ are given by 
        \begin{equation}
            \geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t)= (\diffeo^{-1} \circ\nabla \stroco^\star) ((1 - t)(\nabla \stroco \circ \diffeo)(\Vector) + t (\nabla \stroco \circ \diffeo)(\VectorB)).
            \label{eq:thm-geodesic-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
            \geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t) = \geodesic^\diffeo_{\Vector, \VectorB}(t) = \diffeo^{-1}((1 - t)\diffeo(\Vector) + t \diffeo(\VectorB)).
            \label{eq:thm-geodesic-remetrized-special-psi}
        \end{equation}
        \item the logarithmic map $\log^{\nabla \stroco \circ \diffeo}_{\Vector} (\cdot):\Real^\dimInd \to \tangent_\Vector \Real^\dimInd$  on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        \begin{equation}
            \log^{\nabla \stroco \circ \diffeo}_{\Vector} \VectorB =  D_{\diffeo(\Vector)}\diffeo^{-1}[D_{(\nabla \stroco \circ \diffeo)(\Vector)}\nabla \stroco^\star[(\nabla \stroco \circ \diffeo)(\VectorB) - (\nabla \stroco \circ \diffeo)(\Vector)]].
            \label{eq:thm-log-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
            \log^{\nabla \stroco \circ \diffeo}_{\Vector} \VectorB = \log^\diffeo_{\Vector} \VectorB = D_{\diffeo(\Vector)}\diffeo^{-1}[\diffeo(\VectorB) - \diffeo(\Vector)].
            \label{eq:thm-log-remetrized-special-psi}
        \end{equation}
        \item the exponential map $\exp^{\nabla \stroco \circ \diffeo}_{\Vector} (\cdot):\tangent_\Vector \Real^\dimInd \to \Real^\dimInd$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        \begin{equation}
             \exp^{\nabla \stroco \circ \diffeo}_\Vector (\tangentVector_\Vector) = (\diffeo^{-1} \circ\nabla \stroco^\star)((\nabla \stroco \circ \diffeo)(\Vector) + D_{\diffeo(\Vector)} \nabla \stroco [ D_{\Vector} \diffeo[\tangentVector_\Vector] ]).
             \label{eq:thm-exp-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
             \exp^{\nabla \stroco \circ \diffeo}_\Vector (\tangentVector_\Vector) = \exp^\diffeo_\Vector (\tangentVector_\Vector) = \diffeo^{-1}(\diffeo(\Vector) + D_{\Vector} \diffeo[\tangentVector_\Vector]).
             \label{eq:thm-exp-remetrized-special-psi}
        \end{equation}
        \item the distance $\distance^{\nabla \stroco \circ \diffeo}_{\Real^\dimInd}:\Real^\dimInd \times\Real^\dimInd \to \Real$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        \begin{equation}
            \distance^{\nabla \stroco \circ \diffeo}_{\Real^\dimInd}(\Vector, \VectorB) = \|(\nabla \stroco \circ \diffeo)(\Vector) - (\nabla \stroco \circ \diffeo)(\VectorB)\|_2.
            \label{eq:thm-distance-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
            \distance^{\nabla \stroco \circ \diffeo}_{\Real^\dimInd}(\Vector, \VectorB) = \| \diffeo(\Vector) -  \diffeo(\VectorB)\|_{\spdMatrix^{-2}} := \| \spdMatrix^{-1} (\diffeo(\Vector) -  \diffeo(\VectorB))\|_{2}.
            \label{eq:thm-distance-remetrized-special-psi}
        \end{equation}
        \item the Riemannian barycentre $\Vector^* \in \Real^\dimInd$ of the data set $\{\Vector^\sumIndA\}_{\sumIndA=1}^\dataPointNum$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by
        \begin{equation}
            \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^{\nabla\stroco\circ\diffeo}(\Vector, \Vector^\sumIndA)^2 \Bigr\} = (\diffeo^{-1} \circ\nabla \stroco^\star)\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \nabla \stroco(\diffeo(\Vector^\sumIndA)) \Bigr).
            \label{eq:stroco-diffeo-barycentre-formal}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
            \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^\diffeo(\Vector, \Vector^\sumIndA)^2 \Bigr\} = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr).
            \label{eq:diffeo-barycentre-formal}
        \end{equation}
        % \item parallel transport along geodesics $\mathcal{P}^{\nabla \stroco \circ \diffeo}_{\VectorB \leftarrow \Vector} :\tangent_\Vector \Real^\dimInd \to \tangent_\VectorB \Real^\dimInd$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        % \begin{equation}
        %     \mathcal{P}^{\nabla \stroco \circ \diffeo}_{\VectorB \leftarrow \Vector} \tangentVector_\Vector = D_{\diffeo(\VectorB)}\diffeo^{-1}[D_{(\nabla \stroco \circ \diffeo)(\VectorB)}\nabla \stroco^\star[D_{\diffeo(\Vector)} \nabla \stroco [ D_{\Vector} \diffeo[\tangentVector_\Vector] ] ] ]
        %     \label{eq:thm-parallel-transport-remetrized}
        % \end{equation}
        % In addition, if [psi has form above then]
        % \begin{equation}
        %     \mathcal{P}^{\nabla \stroco \circ \diffeo}_{\VectorB \leftarrow \Vector} \tangentVector_\Vector = \mathcal{P}^\diffeo_{\VectorB \leftarrow \Vector} \tangentVector_\Vector = D_{\diffeo(\VectorB)}\diffeo^{-1} [D_{\Vector} \diffeo[\tangentVector_\Vector] ] 
        %     \label{eq:thm-parallel-transport-remetrized-special-psi}
        % \end{equation}
    \end{enumerate}
\end{proposition}

% Similarly, \cite[Cor.~3.6.1]{diepeveen2024pulling} gives us a closed-form expression of the Riemannian barycentre \citep{karcher1977riemannian} $\Vector^* \in \Real^\dimInd$ of the data set $\{\Vector^\sumIndA\}_{\sumIndA=1}^\dataPointNum$ under $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$
% \begin{equation}
%     \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^{\nabla\stroco\circ\diffeo}(\Vector, \Vector^\sumIndA)^2 \Bigr\} = (\diffeo^{-1} \circ\nabla \stroco^\star)\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \nabla \stroco(\diffeo(\Vector^\sumIndA)) \Bigr),
%     \label{eq:stroco-diffeo-barycentre-formal}
% \end{equation}
% which also simplifies to the barycentre on $(\Real^\dimInd, (\cdot,\cdot)^{\diffeo})$
% \begin{equation}
%     \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^\diffeo(\Vector, \Vector^\sumIndA)^2 \Bigr\} = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr),
%     \label{eq:diffeo-barycentre-formal}
% \end{equation}
% for the special choice of $\stroco$ of the form \cref{eq:quadratic-stroco}.

% Once again, the special case also highlights why we get barycentres in the data support. For instance, in the scenario depicted in \Cref{fig:toy-example-barycentre}, Riemannian barycentre are computed by reversing the effect of the diffeomorphism -- once again transforming the data distribution to a Gaussian -- and then computing the mean of the morphed data points, which is finally mapped back to the original space. Again, this results in a barycentre that lives in the data support.

% \begin{proposition}
% \label{prop:euclidean-diffeo-mean}
%     The barycentre problems \cref{eq:stroco-diffeo-barycentre-formal,eq:diffeo-barycentre-formal} have closed-form solutions given by 
%     \begin{equation}
%         \Vector^* = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr) \quad \text{and}\quad \Vector^* = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr),
%         \label{eq:euclidean-diffeo-mean}
%     \end{equation}
%     which 
% \end{proposition}

% [Add mean as well]

\begin{remark}
\label{rem:stability-manifold-mappings}
    We note that $\ell^2$-stability of geodesics and the barycentre are inherited by \citep[Thms.~3.4\&3.8]{diepeveen2024pulling}, if we have (approximate) local $\ell^2$-isometry of $\diffeo$ on the data distribution.
\end{remark}

\section{Riemannian autoencoder from unimodal probability densities}
\label{sec:rae}

The connection between $(\cdot,\cdot)^{\nabla \stroco \circ \diffeo}$ and $(\cdot,\cdot)^{\diffeo}$ begs the question what $\stroco$ could still be used for if it is of the form \cref{eq:quadratic-stroco}. 
% As an application of the proposed score-based pullback Riemannian geometry, we will show in \Cref{sec:rae-guarantees} that under a specific choice of $\stroco$ there is a natural \emph{Riemannian autoencoder} (RAE) \citep{diepeveen2024pulling} with error bounds, which can be used to retrieve the data manifold like in \Cref{fig:toy-example-manifold}.
We note that this case comes down to having a data probability density that is a deformed Gaussian distribution. In the case of a regular (non-deformed) Gaussian, one can compress the data generated by it through projecting them onto a low rank approximation of the covariance matrix such that only the directions with highest variance are taken into account. This is the basic idea behind PCA. In the following we will generalize this idea to the Riemannian setting and observe that this amounts to constructing a \emph{Riemannian autoencoder} (RAE) \citep{diepeveen2024pulling}, whose error we can bound by picking the dimension of the autoencoder in a clever way, reminiscent of the classical PCA error bound.

Concretely, we assume that we have a unimodal density of the form \cref{eq:stroco-diffeo-density} with a quadratic strongly convex function $\stroco(\Vector):= \frac{1}{2} \Vector^{\top} \spdMatrix^{-1} \Vector$ for some diagonal matrix $\spdMatrix:= \diag(\spdMatrixDiag_1, \ldots \spdMatrixDiag_\dimInd)$ with positive entries\footnote{Note that this is not restrictive as for a general symmetric positive definite matrix $\spdMatrix$ the eigenvalues can be used as diagonal entries and the orthonormal matrices can be concatenated with the diffeomorphism.}. Next, we define an indexing $\coordIndA_\coordIndC \in [\dimInd]:= \{1, \ldots, \dimInd\}$ for $\coordIndC = 1, \ldots, \dimInd$ such that
\begin{equation}
    \spdMatrixDiag_{\coordIndA_1}\geq \ldots \geq \spdMatrixDiag_{\coordIndA_\dimInd},
\end{equation}
and consider a threshold $\RAErelerror\in [0,1]$. We then consider $\dimInd_\RAErelerror \in [\dimInd]$ defined as the integer that satisfies
\begin{equation}
    \dimInd_\RAErelerror := \left\{\begin{matrix}
 \min \Bigl\{ \dimInd'\in [\dimInd-1] \; \Bigl\vert \; \sum_{\coordIndC=\dimInd' + 1}^{\dimInd} \spdMatrixDiag_{\coordIndA_\coordIndC}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA} \Bigr\}, & \text{if } \spdMatrixDiag_{\coordIndA_\dimInd}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA}, \\
 \dimInd, & \text{otherwise.} \\
\end{matrix}\right.  .
\label{eq:dimind-epsilon}
\end{equation}

% \todo{we can make a split between epsilon being large and small for the d is zero case.}
Finally, we define the mapping $\RAEencoder_\RAErelerror:\Real^\dimInd \to \Real^{\dimInd_\RAErelerror}$ coordinate-wise as
\begin{equation}
    \RAEencoder_\RAErelerror(\Vector)_\coordIndC := (\log^\diffeo_{\diffeo^{-1}(\mathbf{0})} \Vector, D_{\mathbf{0}}\diffeo^{-1}[\mathbf{e}^{\coordIndA_\coordIndC}])^\diffeo_{\diffeo^{-1}(\mathbf{0})} \overset{\text{\cref{eq:thm-log-remetrized-special-psi}}}{=} (\diffeo(\Vector), \mathbf{e}^{\coordIndA_\coordIndC})_2, \quad \coordIndC = 1, \ldots, \dimInd_\RAErelerror,
    \label{eq:rae-encoder}
\end{equation}
and define $\RAEdecoder_\RAErelerror:\Real^{\dimInd_\RAErelerror} \to \Real^\dimInd$ as
\begin{equation}
    \RAEdecoder_\RAErelerror(\latentVector):= \exp_{\diffeo^{-1}(\mathbf{0})}^\diffeo \Bigl( \sum_{\coordIndC=1}^{\dimInd_\RAErelerror} \latentVector_\coordIndC D_{\mathbf{0}}\diffeo^{-1}[\mathbf{e}^{\coordIndA_\coordIndC}]\Bigr) \overset{\text{\cref{eq:thm-exp-remetrized-special-psi}}}{=} \diffeo^{-1} \Bigl( \sum_{\coordIndC=1}^{\dimInd_\RAErelerror} \latentVector_\coordIndC \mathbf{e}^{\coordIndA_\coordIndC} \Bigr),
    \label{eq:rae-decoder}
\end{equation}
which generate a Riemannian autoencoder and the set $\RAEdecoder_\RAErelerror(\Real^{\dimInd_\RAErelerror}) \subset \Real^\dimInd$ as an approximate data manifold as in the scenario in \Cref{fig:learned_charts}.

As hinted above, this Riemannian autoencoder comes with an error bound on the expected approximation error, which is fully determined by the diffeomorphism’s deviation from isometry around the data manifold. For the proof, we refer the reader to \Cref{app:proof-of-rae-error}.
\begin{theorem}
\label{thm:rae-error}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a quadratic function of the form \cref{eq:quadratic-stroco} with positive definite diagonal matrix $\spdMatrix \in \Real^{\dimInd\times \dimInd}$. Furthermore, let $\density:\Real^\dimInd \to\Real$ be the corresponding probability density of the form \cref{eq:stroco-diffeo-density}. Finally, consider $\RAErelerror\in [0,1]$ and the mappings $\RAEencoder_\RAErelerror:\Real^\dimInd \to \Real^{\dimInd_\RAErelerror}$ and $\RAEdecoder_\RAErelerror:\Real^{\dimInd_\RAErelerror} \to \Real^\dimInd$ in \cref{eq:rae-encoder,eq:rae-decoder} with $\dimInd_\RAErelerror \in [\dimInd]$ as in \cref{eq:dimind-epsilon}.

    Then, 
    \begin{equation}
        \mathbb{E}_{\stoVector \sim \density}[\| D_\RAErelerror(E_\RAErelerror(\stoVector))-  \stoVector\|_2^2] \leq \RAErelerror \inf_{\RAEboundParam\in [0,\frac{1}{2})}\Bigl\{  \frac{\RAEinvdiffeoRegConstantB \RAEdiffeoRegConstant \RAEinvdiffeoRegConstant}{1 - 2\RAEboundParam} \Bigl(\frac{1 + \RAEboundParam}{1 - 2\RAEboundParam} \Bigr)^{\frac{\dimInd}{2}} \Bigr\} \sum_{\sumIndA=1}^{\dimInd} \spdMatrixDiag_{\sumIndA} + o(\RAErelerror),
        \label{eq:thm-rae-bound}
    \end{equation}
where 
\begin{equation}
    \RAEinvdiffeoRegConstantB := \sup_{\Vector\in \Real^{\dimInd}} \{ \| D_{\diffeo(\Vector)} \diffeo^{-1}\|_2^2 e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \},
    \label{eq:RAEinvdiffeoRegConstantB}
\end{equation}
\begin{equation}
    \RAEdiffeoRegConstant := \sup_{\Vector\in \Real^{\dimInd}} \{ |\det (D_{\Vector} \diffeo)| e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \},
    % \label{eq:RAEdiffeoRegConstant}
\end{equation}
and
\begin{equation}
    \RAEinvdiffeoRegConstant := \sup_{\Vector\in \Real^{\dimInd}} \{ |\det (D_{\diffeo(\Vector)} \diffeo^{-1})| e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \}.
    % \label{eq:RAEinvdiffeoRegConstant}
\end{equation}
\end{theorem}

\begin{remark}
\label{rem:interpretability-rae}
    Note that the RAE latent space is interpretable as it is $\ell^2$-isometric to the data manifold if $\diffeo$ is an approximate $\ell^2$-isometry on the data manifold. In other words, latent representations being close by or far away correspond to similar behaviour in data space, which is not the case for a VAE \citep{kingma2013auto}.
\end{remark}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{../results/banana-distribution/rae_manifold.eps}
%     \caption{For $\RAErelerror = 0.1$ we obtain a Riemannian autoencoder with latent dimension $\dimInd_\RAErelerror = 1$, which yields the manifold in orange.}
%     \label{fig:rae-manifold}
% \end{figure}

==> sections/3-data-analysis.tex <==
\section{Riemannian geometry from unimodal probability densities (2 pages)}
\label{sec:unimodal-riemannian geometry}

\todo{I propose to first define the metric in its most general form from the score, then followed by this section - want to keep this as general as we can for as long as we can.}
In this section we will focus on constructing Riemannian geometry from unimodal densities $\density:\Real^\dimInd\to \Real$ of the form
\begin{equation}
    \density(\Vector) \propto e^{- \stroco(\diffeo(\Vector))}
    \label{eq:stroco-diffeo-density}
\end{equation}
where $\stroco:\Real^\dimInd\to\Real$ is a smooth strongly convex function and $\diffeo:\Real^\dimInd\to\Real^\dimInd$ is a diffeomorphism, e.g., such as the density in \cref{fig:toy-example}\footnote{Here, $\stroco(\Vector) := 2 \Vector_1^2 + \frac{1}{8}\Vector_2^2$ and $\diffeo(\Vector):= (\Vector_1 - \frac{1}{9} \Vector_2^2, \Vector_2)$.}. In particular, we will consider Riemannian structures of the form
\begin{equation}
    (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector} := (D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB])_2,
    \label{eq:stroco-diffeo-pullback}
\end{equation}
which are related to the Riemannian structure obtained from the \emph{score function} $\nabla \log(\density(\cdot)):\Real^\dimInd\to\Real^\dimInd$ if $\diffeo$ is close to a linear $\ell^2$-isometry on the data support:
\begin{multline}
    (D_{\Vector} \nabla \log(\density(\cdot))[\tangentVector], D_{\Vector} \nabla \log(\density(\cdot))[\tangentVectorB])_2 = (D_{\Vector} \nabla (\stroco \circ \diffeo)[\tangentVector], D_{\Vector} \nabla (\stroco \circ \diffeo)[\tangentVectorB])_2 \\
    = (D_{\Vector} ((D_{(\cdot)} \diffeo)^{\top} \circ \nabla\stroco \circ \diffeo)[\tangentVector], D_{\Vector}((D_{(\cdot)} \diffeo)^{\top} \circ \nabla\stroco \circ \diffeo) [\tangentVectorB])_2 \\
    \approx (D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB])_2 = (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector}.
\end{multline}

The main motivation for considering Riemannian structures of the form \cref{eq:stroco-diffeo-pullback} rather than ones obtained from the score itself comes from the fact that $\nabla \stroco \circ \diffeo$ is a diffeomorphism. This allows to construct pullback geometry such that geodesics and other manifold mappings behave like in \cref{fig:toy-example-barycentre,fig:toy-example-geodesic,fig:toy-example-log,fig:toy-example-exp} -- as is to be expected from Riemannian structures based of the score \cite{sorrenson2024learningdistancesdatanormalizing} --, which will be discussed in \cref{sec:manifold-mappings}. Subsequently, from the observations in \cref{sec:manifold-mappings} we will show in \cref{sec:rae-guarantees} that under a specific choice of $\stroco$ there is a natural Riemannian autoencoder (RAE) with error bounds, which can be used to retrieve the data manifold like in \cref{fig:toy-example-manifold}.\todo{I will need some help in understanding exactly what you are talking about here - why does the RAE appear?}


\subsection{Manifold mappings}
\label{sec:manifold-mappings}

The following result, which is a direct application of \cite[Prop.~2.1]{diepeveen2024pulling}, gives us closed-form expressions of several important manifold mappings under $(\cdot,\cdot)^{\nabla \stroco \circ \diffeo}$ and makes a connection with $(\cdot,\cdot)^{\diffeo}$ if we choose
\begin{equation}
    \stroco(\Vector)=\frac{1}{2} \Vector^{\top} \spdMatrix^{-1} \Vector,
    \label{eq:quadratic-stroco}
\end{equation}
where $\spdMatrix\in \Real^{\dimInd\times \dimInd}$ is symmetric positive definite. 

% This special case also makes it especially clear why we also in general get geodesics and manifold mappings that go through the data support. For example, in the case of \cref{fig:toy-example}, which has the correct form \cref{eq:stroco-diffeo-density}, geodesics are just computed by undoing the effect of the diffeomporphism first -- so that the data distribution looks like a Gaussian -- and then computing straight lines between the data points. This will result in geodesics that move through regions with higher likelihoods than the end points, because of the strong convexity of the quadratic function, which is exactly what we want.

This special case highlights why, in general, we obtain geodesics and manifold mappings that pass through the data support. For instance, in the scenario depicted in \cref{fig:toy-example-geodesic}, where the correct form \cref{eq:stroco-diffeo-density} is used, geodesics are computed by first reversing the effect of the diffeomorphism -- transforming the data distribution to resemble a Gaussian --, then drawing straight lines between the morphed data points, and finally applying the diffeomorphism again. This approach results in geodesics that traverse regions of higher likelihood between the endpoints, due to the strong convexity of the quadratic function, which aligns perfectly with our objectives.
\todo{I have a question: why does this need to be presented as composition of sc and diffeo, if the result is effectively for just diffeo?}
\begin{proposition}
\label{thm:pull-back-mappings}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a smooth strongly convex function, whose Fenchel conjugate is denoted by $\stroco^\star: \Real^\dimInd\to\Real$. Next, consider the $\ell^2$-pullback manifolds $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ and $(\Real^\dimInd, (\cdot,\cdot)^{\diffeo})$ defined through metric tensor fields
    \begin{equation}
        (\tangentVector, \tangentVectorB)^{\nabla \stroco \circ \diffeo}_{\Vector} := (D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVector], D_{\Vector} \nabla \stroco \circ \diffeo[\tangentVectorB])_2, \quad \text{and} \quad (\tangentVector, \tangentVectorB)^{\diffeo}_{\Vector} := (D_{\Vector} \diffeo[\tangentVector], D_{\Vector} \diffeo[\tangentVectorB])_2.
    \end{equation}

    Then,
    \begin{enumerate}[label=(\roman*)]
        \item length-minimising geodesics $\geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}:[0,1] \to \Real^\dimInd$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ are given by 
        \begin{equation}
            \geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t)= (\diffeo^{-1} \circ\nabla \stroco^*) ((1 - t)(\nabla \stroco \circ \diffeo)(\Vector) + t (\nabla \stroco \circ \diffeo)(\VectorB)).
            \label{eq:thm-geodesic-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
            \geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t) = \geodesic^\diffeo_{\Vector, \VectorB}(t) = \diffeo^{-1}((1 - t)\diffeo(\Vector) + t \diffeo(\VectorB)).
            \label{eq:thm-geodesic-remetrized-special-psi}
        \end{equation}
        \item the logarithmic map $\log^{\nabla \stroco \circ \diffeo}_{\Vector} (\cdot):\Real^\dimInd \to \tangent_\Vector \Real^\dimInd$  on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        \begin{equation}
            \log^{\nabla \stroco \circ \diffeo}_{\Vector} \VectorB =  D_{\diffeo(\Vector)}\diffeo^{-1}[D_{(\nabla \stroco \circ \diffeo)(\Vector)}\nabla \stroco^*[(\nabla \stroco \circ \diffeo)(\VectorB) - (\nabla \stroco \circ \diffeo)(\Vector)]]
            \label{eq:thm-log-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
            \log^{\nabla \stroco \circ \diffeo}_{\Vector} \VectorB = \log^\diffeo_{\Vector} \VectorB = D_{\diffeo(\Vector)}\diffeo^{-1}[\diffeo(\VectorB) - \diffeo(\Vector)]
            \label{eq:thm-log-remetrized-special-psi}
        \end{equation}
        \item the exponential map $\exp^{\nabla \stroco \circ \diffeo}_{\Vector} (\cdot):\tangent_\Vector \Real^\dimInd \to \Real^\dimInd$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        \begin{equation}
             \exp^{\nabla \stroco \circ \diffeo}_\Vector (\tangentVector_\Vector) = (\diffeo^{-1} \circ\nabla \stroco^*)((\nabla \stroco \circ \diffeo)(\Vector) + D_{\diffeo(\Vector)} \nabla \stroco [ D_{\Vector} \diffeo[\tangentVector_\Vector] ])
             \label{eq:thm-exp-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
             \exp^{\nabla \stroco \circ \diffeo}_\Vector (\tangentVector_\Vector) = \exp^\diffeo_\Vector (\tangentVector_\Vector) = \diffeo^{-1}(\diffeo(\Vector) + D_{\Vector} \diffeo[\tangentVector_\Vector])
             \label{eq:thm-exp-remetrized-special-psi}
        \end{equation}
        \item the distance $\distance^{\nabla \stroco \circ \diffeo}_{\Real^\dimInd}:\Real^\dimInd \times\Real^\dimInd \to \Real$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        \begin{equation}
            \distance^{\nabla \stroco \circ \diffeo}_{\Real^\dimInd}(\Vector, \VectorB) = \|(\nabla \stroco \circ \diffeo)(\Vector) - (\nabla \stroco \circ \diffeo)(\VectorB)\|_2,
            \label{eq:thm-distance-remetrized}
        \end{equation}
        In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco}
        \begin{equation}
            \distance^{\nabla \stroco \circ \diffeo}_{\Real^\dimInd}(\Vector, \VectorB) = \| \diffeo(\Vector) -  \diffeo(\VectorB)\|_{\spdMatrix^{-2}} := \| \spdMatrix^{-1} (\diffeo(\Vector) -  \diffeo(\VectorB))\|_{2},
            \label{eq:thm-distance-remetrized-special-psi}
        \end{equation}
        % \item parallel transport along geodesics $\mathcal{P}^{\nabla \stroco \circ \diffeo}_{\VectorB \leftarrow \Vector} :\tangent_\Vector \Real^\dimInd \to \tangent_\VectorB \Real^\dimInd$ on $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$ is given by 
        % \begin{equation}
        %     \mathcal{P}^{\nabla \stroco \circ \diffeo}_{\VectorB \leftarrow \Vector} \tangentVector_\Vector = D_{\diffeo(\VectorB)}\diffeo^{-1}[D_{(\nabla \stroco \circ \diffeo)(\VectorB)}\nabla \stroco^*[D_{\diffeo(\Vector)} \nabla \stroco [ D_{\Vector} \diffeo[\tangentVector_\Vector] ] ] ]
        %     \label{eq:thm-parallel-transport-remetrized}
        % \end{equation}
        % In addition, if [psi has form above then]
        % \begin{equation}
        %     \mathcal{P}^{\nabla \stroco \circ \diffeo}_{\VectorB \leftarrow \Vector} \tangentVector_\Vector = \mathcal{P}^\diffeo_{\VectorB \leftarrow \Vector} \tangentVector_\Vector = D_{\diffeo(\VectorB)}\diffeo^{-1} [D_{\Vector} \diffeo[\tangentVector_\Vector] ] 
        %     \label{eq:thm-parallel-transport-remetrized-special-psi}
        % \end{equation}
    \end{enumerate}
\end{proposition}

Similarly, \cite[Cor.~3.6.1]{diepeveen2024pulling} gives us a closed-form expression of the Riemannian barycentre \cite{karcher1977riemannian} $\Vector^* \in \Real^\dimInd$ of the data set $\{\Vector^\sumIndA\}_{\sumIndA=1}^\dataPointNum$ under $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$
\begin{equation}
    \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^{\nabla\stroco\circ\diffeo}(\Vector, \Vector^\sumIndA)^2 \Bigr\} = (\diffeo^{-1} \circ\nabla \stroco^*)\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \nabla \stroco(\diffeo(\Vector^\sumIndA)) \Bigr),
    \label{eq:stroco-diffeo-barycentre-formal}
\end{equation}
which also simplifies to the barycentre on $(\Real^\dimInd, (\cdot,\cdot)^{\diffeo})$
\begin{equation}
    \Vector^* := \argmin_{\Vector\in \Real^\dimInd} \Bigl\{ \frac{1}{2\dataPointNum}\sum_{\sumIndA = 1}^\dataPointNum \distance_{\Real^\dimInd}^\diffeo(\Vector, \Vector^\sumIndA)^2 \Bigr\} = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr),
    \label{eq:diffeo-barycentre-formal}
\end{equation}
for the special choice of $\stroco$ of the form \cref{eq:quadratic-stroco}.

Once again, the special case also highlights why we get barycentres in the data support. For instance, in the scenario depicted in \cref{fig:toy-example-barycentre}, Riemannian barycentre are computed by reversing the effect of the diffeomorphism -- once again transforming the data distribution to a Gaussian -- and then computing the mean of the morphed data points, which is finally mapped back to the original space. Again, this results in a barycentre that lives in the data support.

% \begin{proposition}
% \label{prop:euclidean-diffeo-mean}
%     The barycentre problems \cref{eq:stroco-diffeo-barycentre-formal,eq:diffeo-barycentre-formal} have closed-form solutions given by 
%     \begin{equation}
%         \Vector^* = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr) \quad \text{and}\quad \Vector^* = \diffeo^{-1}\Bigl(\frac{1}{\dataPointNum} \sum_{\sumIndA=1}^\dataPointNum \diffeo(\Vector^\sumIndA) \Bigr),
%         \label{eq:euclidean-diffeo-mean}
%     \end{equation}
%     which 
% \end{proposition}

% [Add mean as well]

\begin{remark}
    We note that stability of geodesics and the barycentre are inherited by \cite[Thms.~3.4\&3.8]{diepeveen2024pulling}, if we have (approximate) local $\ell^2$-isometry of $\diffeo$ on the data distribution.
\end{remark}

\subsection{Riemannian autoencoder}
\label{sec:rae-guarantees}

The special case of having a quadratic strongly convex function comes down to having a data probability density that is a deformed Gaussian distribution. In the case of a regular (non-deformed) Gaussian, one can compress the data generated by it through projecting them onto a low rank approximation of the covariance matrix such that only the directions with highest variance are taken into account. In the following we will generalize this idea to the Riemannian setting and observe that this amounts to constructing a Riemannian autoencoder \cite{diepeveen2024pulling}, whose error we can bound by picking the dimension of the autoencoder in a clever way.

We assume that we have a unimodal density of the form \cref{eq:stroco-diffeo-density} with a quadratic strongly convex function $\stroco(\Vector):= \frac{1}{2} \Vector^{\top} \spdMatrix^{-1} \Vector$ for some diagonal matrix $\spdMatrix:= \diag(\spdMatrixDiag_1, \ldots \spdMatrixDiag_\dimInd)$ with positive entries\footnote{Note that this is not restrictive as for a general symmetric positive definite matrix $\spdMatrix$ the eigenvalues can be used as diagonal entries and the orthonormal matrices can be concatenated with the diffeomorphism.}. Next, we define an indexing $\coordIndA_\coordIndC \in [\dimInd]:= \{1, \ldots, \dimInd\}$ for $\coordIndC = 1, \ldots, \dimInd$ such that
\begin{equation}
    \spdMatrixDiag_{\coordIndA_1}\geq \ldots \geq \spdMatrixDiag_{\coordIndA_\dimInd},
\end{equation}
and consider a threshold $\RAErelerror\in [0,1]$. We then consider $\dimInd_\RAErelerror \in [\dimInd]$ defined as the integer that satisfies
\begin{equation}
    \dimInd_\RAErelerror := \left\{\begin{matrix}
 \min \Bigl\{ \dimInd'\in [\dimInd-1] \; \Bigl\vert \; \sum_{\coordIndC=\dimInd' + 1}^{\dimInd} \spdMatrixDiag_{\coordIndA_\coordIndC}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA} \Bigr\}, & \text{if } \spdMatrixDiag_{\coordIndA_\dimInd}  \leq \RAErelerror \sum_{\coordIndA=1}^{\dimInd} \spdMatrixDiag_{\coordIndA}, \\
 \dimInd, & \text{otherwise.} \\
\end{matrix}\right.  .
\label{eq:dimind-epsilon}
\end{equation}

% \todo{we can make a split between epsilon being large and small for the d is zero case.}
Finally, we define the mapping $\RAEencoder_\RAErelerror:\Real^\dimInd \to \Real^{\dimInd_\RAErelerror}$ coordinate-wise as
\begin{equation}
    \RAEencoder_\RAErelerror(\Vector)_\coordIndC := (\log^\diffeo_{\diffeo^{-1}(\mathbf{0})} \Vector, D_{\mathbf{0}}\diffeo^{-1}[\mathbf{e}^{\coordIndA_\coordIndC}])^\diffeo_{\diffeo^{-1}(\mathbf{0})} \overset{\text{\cref{eq:thm-log-remetrized-special-psi}}}{=} (\diffeo(\Vector), \mathbf{e}^{\coordIndA_\coordIndC})_2, \quad \coordIndC = 1, \ldots, \dimInd_\RAErelerror,
    \label{eq:rae-encoder}
\end{equation}
and define $\RAEdecoder_\RAErelerror:\Real^{\dimInd_\RAErelerror} \to \Real^\dimInd$ as
\begin{equation}
    \RAEdecoder_\RAErelerror(\latentVector):= \exp_{\diffeo^{-1}(\mathbf{0})}^\diffeo \Bigl( \sum_{\coordIndC=1}^{\dimInd_\RAErelerror} \latentVector_\coordIndC D_{\mathbf{0}}\diffeo^{-1}[\mathbf{e}^{\coordIndA_\coordIndC}]\Bigr) \overset{\text{\cref{eq:thm-exp-remetrized-special-psi}}}{=} \diffeo^{-1} \Bigl( \sum_{\coordIndC=1}^{\dimInd_\RAErelerror} \latentVector_\coordIndC \mathbf{e}^{\coordIndA_\coordIndC} \Bigr),
    \label{eq:rae-decoder}
\end{equation}
which generate a Riemannian autoencoder and from which the data manifold can be retrieved as in the scenario in \cref{fig:toy-example-manifold}.

In addition, this Riemannian autoencoder comes with an error bound on the expected approximation error, which is fully determined by the diffeomorphism’s deviation from isometry around the data manifold. For the proof, we refer the reader to \cref{app:proof-of-rae-error}.
\begin{theorem}
\label{thm:rae-error}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a quadratic function of the form \cref{eq:quadratic-stroco} with diagonal $\spdMatrix \in \Real^{\dimInd\times \dimInd}$. Furthermore, let $\density:\Real^\dimInd \to\Real$ be the corresponding probability density of the form \cref{eq:stroco-diffeo-density}. Finally, consider $\RAErelerror\in [0,1]$ and the mappings $\RAEencoder_\RAErelerror:\Real^\dimInd \to \Real^{\dimInd_\RAErelerror}$ and $\RAEdecoder_\RAErelerror:\Real^{\dimInd_\RAErelerror} \to \Real^\dimInd$ in \cref{eq:rae-encoder,eq:rae-decoder} with $\dimInd_\RAErelerror \in [\dimInd]$ as in \cref{eq:dimind-epsilon}.

    Then, 
    \begin{equation}
        \mathbb{E}_{\stoVector \sim \density}[\| D_\RAErelerror(E_\RAErelerror(\stoVector))-  \stoVector\|_2^2] \leq \RAErelerror \inf_{\RAEboundParam\in [0,\frac{1}{2})}\Bigl\{  \frac{\RAEinvdiffeoRegConstantB \RAEdiffeoRegConstant \RAEinvdiffeoRegConstant}{1 - 2\RAEboundParam} \Bigl(\frac{1 + \RAEboundParam}{1 - 2\RAEboundParam} \Bigr)^{\frac{\dimInd}{2}} \Bigr\} \sum_{\sumIndA=1}^{\dimInd} \spdMatrixDiag_{\sumIndA} + o(\RAErelerror),
        \label{eq:thm-rae-bound}
    \end{equation}
where 
\begin{equation}
    \RAEinvdiffeoRegConstantB := \sup_{\Vector\in \Real^{\dimInd}} \{ \| D_{\diffeo(\Vector)} \diffeo^{-1}\|_2^2 e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \},
    \label{eq:RAEinvdiffeoRegConstantB}
\end{equation}
\begin{equation}
    \RAEinvdiffeoRegConstant := \sup_{\Vector\in \Real^{\dimInd}} \{ |\det (D_{\diffeo(\Vector)} \diffeo^{-1})| e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \},
    % \label{eq:RAEinvdiffeoRegConstant}
\end{equation}
and
\begin{equation}
    \RAEdiffeoRegConstant := \sup_{\Vector\in \Real^{\dimInd}} \{ |\det (D_{\Vector} \diffeo)| e^{-\frac{\RAEboundParam}{2} \diffeo(\Vector)^\top \spdMatrix^{-1} \diffeo(\Vector) } \}.
    % \label{eq:RAEdiffeoRegConstant}
\end{equation}
\end{theorem}

\begin{remark}
    Note that the RAE latent space is interpretable as it is isometric to the data manifold if $\diffeo$ is an approximate $\ell^2$-isometry. In other words, latent representations being close by or far away correspond to similar behaviour in data space, which is not the case for a VAE \cite{kingma2013auto}.
\end{remark}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{../results/banana-distribution/rae_manifold.eps}
%     \caption{For $\RAErelerror = 0.1$ we obtain a Riemannian autoencoder with latent dimension $\dimInd_\RAErelerror = 1$, which yields the manifold in orange.}
%     \label{fig:rae-manifold}
% \end{figure}

==> sections/4-score-based-learning.tex <==
\section{Learning unimodal probability densities }
\label{sec:adapting-normalizing-flows}
% - Next, we know what type of unimodal distribution is ideal for downstream data processing, we construct a learning problem for it that incorporates the lessons learnt, i.e., we need $\ell^2$-isometry on the data manifold

Naturally, we want to learn probability densities of the form \cref{eq:stroco-diffeo-density}, which can then directly be inserted into the proposed score-based pullback Riemannian geometry framework. In this section we will consider how to adapt normalizing flow (NF) \citep{dinh2017density} training to a setting that is more suitable for our purposes\footnote{We note that the choice for adapting the normalizing flow training scheme rather than using diffusion model training schemes is due to more robust results through the former.}. In particular, we will consider how training a normalizing flow density $\density: \Real^\dimInd\to\Real$ given by 
\begin{equation}
    \density(\Vector):= \frac{1}{C_{\stroco}}e^{- \stroco(\diffeo(\Vector))} |\det(D_{\Vector} \diffeo)|,
    \label{eq:nf-density}
\end{equation}
where $C_{\stroco}>0$ is a normalisation constant that only depends on the strongly convex function $\stroco$, yields our target distribution \cref{eq:stroco-diffeo-density}.

From \Cref{sec:unimodal-riemannian geometry,sec:rae} we have seen that ideally the strongly convex function $\stroco: \Real^{\dimInd} \to \Real$ corresponds to a Gaussian with a parameterised diagonal covariance matrix $\spdMatrix \in \Real^{\dimInd\times \dimInd}$, resulting in more parameters than in standard normalizing flows, whereas the diffeomorphism $\diffeo: \Real^{\dimInd} \to \Real^{\dimInd}$ is regularized to be an isometry. In particular, $\spdMatrix$ ideally allows for learnable anisotropy rather than having a fixed isotropic identity matrix. The main reason is that through anisotropy we can construct a Riemannian autoencoder (RAE), since it is known which dimensions are most important. Moreover, the diffeomorphism should be $\ell^2$-isometric, unlike standard normalizing flows which are typically non-volume preserving, enabling stability (\Cref{rem:stability-manifold-mappings}) and a practically useful and interpretable RAE  (\Cref{thm:rae-error,rem:interpretability-rae}). In addition, $\ell^2$-isometry (on the data support) implies volume-preservation, which means that $|\det(D_{\Vector} \diffeo)| \approx 1$ so that \cref{eq:nf-density} reduces to the target distribution \cref{eq:stroco-diffeo-density}\footnote{We note that without these constraints (accommodating multimodality) the learned mappings can in principle be used to construct Riemannian geometry and a RAE. However, from the theory discussed in this paper we cannot guarantee stability of manifold mappings nor that the RAE has the right dimension.}.

% - say that our approach will rely on normalizing flow training. However, from the sections above, we have seen that we might want to change some things. The main considerations for constructing useful and stable Riemannian geometry
% -- not just volume preserving diffeomorphisms, but ell2 isometries for stability of geodesics and an interpretable RAE. This is a stronger requirement
% -- anisotropic prior to construct the RAE in the first place

% These observations should be reflected in our parametrisation and subsequent learning scheme. For that consider a data set $(\Vector^\sumIndA)_{\sumIndA=1}^\dataPointNum$, whose density we aim to learn, and let $\mu:= \frac{1}{\dataPointNum}\sum_{\sumIndA=1}^\dataPointNum \Vector^\sumIndA$ be the empirical mean of the data and $\mathbf{Q}\Lambda \mathbf{Q}^\top:= \frac{1}{\dataPointNum-1}\sum_{\sumIndA=1}^\dataPointNum (\Vector^\sumIndA - \mu)  (\Vector^\sumIndA - \mu)^\top$ be the eigendecompisition of the empirical data variance. [Regarding parametrisation, we consider]
% \begin{equation}
%     \stroco_{\networkParams_1} (\Vector):= \frac{1}{2}[] , \quad \diffeo_{\networkParams_2}(\Vector):= \diffeoB \circ   
% \end{equation}

% - parametrisation + initialisation
% -- as we have seen that the we want to train deformed Gaussians, it makes sense to initialize with a linear Gaussian approximation. So we consider invertible neural networks of the form
% -- rational quadratic flows \cite{durkan2019neural}
% -- softplus

% - loss
% -- normalizing flow loss
% -- isometry 
% -- possible loss on trace of A

This leads to learning the density through minimizing the following adapted normalizing flow loss
\begin{multline}\label{eq:basic_training_objective}
    \mathcal{L}(\networkParams_1, \networkParams_2) := \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[-\log \density_{\networkParams_1, \networkParams_2}(\stoVector)\right] \\
    + \lambda_{\text{vol}} \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[ \log(|\det \bigl( D_{\stoVector} \diffeo_{\networkParams_2} \bigr)|)^2 \right] \\
    +
    \lambda_{\text{iso}} \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[ \|  (D_{\stoVector} \diffeo_{\networkParams_2})^\top D_{\stoVector} \diffeo_{\networkParams_2}  - \mathbf{I}_\dimInd\|_F^2 \right]
    % \lambda_{\text{iso}} \mathbb{E}_{\stoVector \sim \density_{\text{data}}, \eta\sim \mathcal{N}(\mathbf{0}, \mathbf{I})}\left[(\| (D_{\stoVector} \diffeo_{\networkParams_2})^*\eta\|_2^2 - \|\eta\|_2^2)^2\right] 
\end{multline}
where $\lambda_{\text{vol}}, \lambda_{\text{iso}} >0$ and the negative log likelihood term reduces to
\begin{multline}
    \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[-\log \density_{\networkParams_1, \networkParams_2}(\stoVector)\right] 
    = \frac{1}{2}\mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[\diffeo_{\networkParams_2}(\stoVector)^\top \spdMatrix_{\networkParams_1}^{-1} \diffeo_{\networkParams_2}(\stoVector) \right] \\
    - \mathbb{E}_{\stoVector \sim \density_{\text{data}}}\left[ \log(|\det \bigl( D_{\stoVector} \diffeo_{\networkParams_2} \bigr)|) \right] + \frac{1}{2} \trace(\log(\spdMatrix_{\networkParams_1})) + \frac{\dimInd}{2}\log(2\pi),
\end{multline}
where $\spdMatrix_{\networkParams_1}$ is a diagonal matrix and $\diffeo_{\networkParams_2}$ is a normalizing flow with affine coupling layers\footnote{We note that the choice for affine coupling layers rather than using more expressive diffeomorphisms such as rational quadratic flows \cite{durkan2019neural} is due to our need for high regularity for stable manifold mappings (\Cref{rem:stability-manifold-mappings}) and an interpretable RAE (\Cref{rem:interpretability-rae}), which has empirically shown to be more challenging to achieve for more expressive flows as both first-and higher-order derivatives of $\diffeo$ will blow up the error terms in \cref{thm:rae-error}. For more details refer to \cref{app:Experiments-with-more-complex-distributions}.
} \citep{dinh2017density}. 
% [remark about initialization]

% \begin{remark}
%     Given the connection between PCA and the RAE discussed in \Cref{sec:rae}, it is reasonable to attempt using PCA for initialization. In particular, given a data set $(\Vector^\sumIndA)_{\sumIndA=1}^\dataPointNum$ this would amount to choosing $\spdMatrix_{\networkParams_1^0}:= \Lambda$ and $\diffeo_{\networkParams_2^0}:= \diffeoB_{\networkParams_2^0}\circ\mathbf{U}^\top \circ (\cdot - \mu)$, where 
%     \begin{equation}
%         \mathbf{U}\Lambda\mathbf{U}^\top = \frac{1}{\dataPointNum-1}\sum_{\sumIndA=1}^\dataPointNum (\Vector^\sumIndA - \mu)  (\Vector^\sumIndA - \mu)^\top
%     \end{equation}
%     is the eigendecomposition of the empirical data variance with $\mu:= \frac{1}{\dataPointNum}\sum_{\sumIndA=1}^\dataPointNum \Vector^\sumIndA$ and $\diffeoB_{\networkParams_2^0}$ is a rational quadratic flow initialized close to identity. However, we note that in practice this might not always yield favorable outcomes. For instance, after applying the rotation matrix $\mathbf{U}$ to image data, using efficient network architectures like CNNs to estimate the rational quadratic flow coefficients becomes less intuitive.
% \end{remark}

==> sections/5-numerics.tex <==
\section{Experiments}
\label{sec:numerics}

We conducted two sets of experiments to evaluate the proposed scheme from \Cref{sec:adapting-normalizing-flows} to learn suitable pullback Riemannian geometry. The first set investigates whether our adaptation of the standard normalizing flow (NF) training paradigm leads to more accurate and stable manifold mappings, as measured by the geodesic and variation errors. The second set assesses the capability of our method to generate a robust Riemannian autoencoder (RAE).

For all experiments in this section, detailed training configurations are provided in \Cref{app:training_details}.


%We found that our proposed training paradigm not only provides more stable and accurate manifold mappings but also effectively serves as a Riemannian autoencoder. The learned variances of the base distribution \(\spdMatrix_{\networkParams_1}\) capture the variance in both on-manifold and off-manifold directions. Specifically, high learned variances correspond to on-manifold directions (directions along the manifold), while small variances correspond to off-manifold directions (directions orthogonal to the manifold).

%In the our Riemannian auto-encoder, the encoder maps a data point \(x\) to its latent representation \(z = \phi(x)\), where \(\phi\) is the learned diffeomorphism. We retain the components of \(z\) corresponding to high variances, as indicated by \(\spdMatrix_{\networkParams_1}\), and discard the components corresponding to low variances. The decoder reconstructs the data by setting the discarded components of \(z\) to zero to obtain \(\hat{z}\), and then applying the inverse transformation \(\phi^{-1}(\hat{z})\).

\subsection{Manifold mappings}
\label{sec:manifold-mappings-experiments}

As discussed in \citet{diepeveen2024pulling}, the quality of learned manifold mappings is determined by two key metrics: the \emph{geodesic error} and the \emph{variation error}. The geodesic error measures the average deviation form the ground truth geodesics implied by the ground truth pullback metric, while the variation error evaluates the stability of geodesics under small perturbations. We define these error metrics for the evaluation of pullback geometries in Appendix \ref{app:Error metrics for evaluation of Pullback Geometries}.

Our approach introduces two key modifications to the normalizing flow (NF) training framework:

\begin{enumerate}
    \item \textbf{Anisotropic Base Distribution}: We parameterize the diagonal elements of the covariance matrix \(\spdMatrix_{\networkParams_1}\), introducing anisotropy into the base distribution.
    
    \item \textbf{\(\ell^2\)-Isometry Regularization}: We regularize the flow \(\diffeo_{\networkParams_2}\) to be approximately \(\ell^2\)-isometric.
\end{enumerate}

To assess the effectiveness of these modifications in learning more accurate and robust manifold mappings, we compare our method against three baselines:

\begin{enumerate}[label=(\arabic*)]
    \item \emph{Normalizing Flow (NF)}: Uses an NF with a standard isotropic Gaussian base distribution $\mathcal{N}(\mathbf{0}, \mathbf{I}_\dimInd)$ and no isometry regularization of the flow.
    \item \emph{Anisotropic Normalizing Flow}: Uses an NF with the same parameterization of the diagonal covariance matrix in the base distribution as in our method, but without regularization of the flow.
    \item \emph{Isometric Normalizing Flow}: Uses an NF with an isotropic Gaussian base distribution $\mathcal{N}(\mathbf{0}, \mathbf{I}_\dimInd)$ and regularizes the flow to be approximately $\ell^2$-isometric.
\end{enumerate}

We conduct experiments on three datasets, illustrated in \Cref{fig:datasets} in \Cref{app:manifold_mapping}: the \emph{Single Banana Dataset}, the \emph{Squeezed Single Banana Dataset}, and the \emph{River Dataset}. Detailed descriptions of the construction and characteristics of these datasets are provided in \Cref{app:manifold_mapping}.

\Cref{tab:geodesic-variation-errors} presents the geodesic and variation errors for each method across the three datasets and \Cref{fig:geodesics_comparison} visually compares the geodesics computed using each method on the river dataset. Our method consistently achieves significantly lower errors compared to the baselines, indicating more accurate and stable manifold mappings. 

Introducing anisotropy in the base distribution without enforcing isometry in the flow offers no significant improvement over the standard flow. On the other hand, regularizing the flow to be approximately isometric without incorporating anisotropy in the base distribution results in underfitting, leading to noticeably worse performance than the standard flow. Our results demonstrate that the combination of anisotropy in the base distribution with isometry regularization (our method) yields the most accurate and stable manifold mappings, as evidenced by consistently lower geodesic and variation errors.

\begin{table}[t!]
\centering
\begin{tabular}{lcccc}
\hline
\textbf{Metric} & \textbf{Our Method} & \textbf{NF} & \textbf{Anisotropic NF} & \textbf{Isometric NF} \\
\hline
\multicolumn{5}{c}{\textbf{Single Banana Dataset}} \\
\hline
Geodesic Error & \textbf{0.0315 (0.0268)} & 0.0406 (0.0288) & 0.0431 (0.0305) & 0.0817 (0.1063) \\
Variation Error & \textbf{0.0625 (0.0337)} & 0.0638 (0.0352) & 0.0639 (0.0354) & 0.0639 (0.0355) \\
\hline
\multicolumn{5}{c}{\textbf{Squeezed Single Banana Dataset}} \\
\hline
Geodesic Error & \textbf{0.0180 (0.0226)} & 0.0524 (0.0805) & 0.0505 (0.0787) & 0.1967 (0.2457) \\
Variation Error & \textbf{0.0631 (0.0326)} & 0.0663 (0.0353) & 0.0661 (0.0350) & 0.0669 (0.0361) \\
\hline
\multicolumn{5}{c}{\textbf{River Dataset}} \\
\hline
Geodesic Error & \textbf{0.1691 (0.0978)} & 0.2369 (0.1216) & 0.2561 (0.1338) & 0.3859 (0.2568) \\
Variation Error & \textbf{0.0763 (0.0486)} & 0.1064 (0.0807) & 0.1113 (0.0863) & 0.0636 (0.0333) \\
\hline
\end{tabular}
\caption{Comparison of evaluation metrics for different methods across three datasets. Best-performing results for each metric are highlighted in bold. Values are reported as mean (std). The proposed method performs best in all metrics on each data set.}
\label{tab:geodesic-variation-errors}
\end{table}

\begin{figure}[htbp]
\centering
\begin{subfigure}[b]{0.195\textwidth}
\includegraphics[width=\textwidth]{results/visualisations/geodesics/gt.png}
\caption{Ground Truth}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
\includegraphics[width=\textwidth]{results/visualisations/geodesics/ours.png}
\caption{Our Method}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
\includegraphics[width=\textwidth]{"results/visualisations/geodesics/standard_normal.png"}
\caption{Standard NF}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
\includegraphics[width=\textwidth]{"results/visualisations/geodesics/standard_normal_anisotropic.png"}
\caption{Anisotropic NF}
\end{subfigure}
\begin{subfigure}[b]{0.195\textwidth}
\includegraphics[width=\textwidth]{results/visualisations/geodesics/isometricNF.png}
\caption{Isometric NF}
\end{subfigure}
\caption{Comparison of geodesics computed using different methods on the river dataset. The geodesics generated by the proposed method have least artifacts, which is in line with our expectations from Table~\ref{tab:geodesic-variation-errors}.}
\label{fig:geodesics_comparison}
\end{figure}



\subsection{Riemannian autoencoder}
\label{sec:RAE-experiments}
To evaluate the capacity of our method to learn a Riemannian autoencoder, we conducted experiments on two synthetic datasets across various combinations of intrinsic dimension $\dimInd'$ and ambient dimension $\dimInd$:

\begin{itemize}
    \item \textit{Hemisphere}($\dimInd'$, $\dimInd$): Samples are drawn from the upper hemisphere of a $\dimInd'$-dimensional unit sphere and embedded in an $\dimInd$-dimensional ambient space via a random isometric mapping.
    \item \textit{Sinusoid}($\dimInd'$, $\dimInd$): This dataset is generated by applying sinusoidal transformations to $\dimInd'$-dimensional latent variables, resulting in a complex, nonlinear manifold embedded in $\dimInd$ dimensions.
\end{itemize}

For a detailed description of these datasets, refer to \Cref{app:rae_datasets}.

% \subsection{Results}

\subsubsection{1D and 2D manifolds}
In \Cref{fig:learned_charts,fig:learned_charts_for_Sinusoid_1_100}, we present the data manifold approximations by our Riemannian autoencoder for four low-dimensional manifolds.: Hemisphere(2,3), Sinusoid(1,3), Sinusoid(2,3) and Sinusoid(1,100). In \cref{app:data_manifold_approximation}, we detail the process used to create the data manifold approximations for these experiments. In our experiments, we set \( \epsilon = 0.01 \), which resulted in \( d_{\epsilon} = \dimInd' \) for all cases, accurately capturing the intrinsic dimension of each manifold and producing accurate global charts.






% \begin{figure}[htb]
%     \centering

%     % First row: Projections of RAE for three datasets
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{results/visualisations/RAE/projections/hemisphere_2_3/riemannian_autoencoder.jpg}
%         \caption{Hemisphere (2,3)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{results/visualisations/RAE/projections/sinusoid_1_3/riemannian_autoencoder.jpg}
%         \caption{Sinusoid (1,3)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{results/visualisations/RAE/projections/sinusoid_2_3/riemannian_autoencoder.jpg}
%         \caption{Sinusoid (2,3)}
%     \end{subfigure}

%     \caption{
%         Approximate data manifolds learned by the Riemannian autoencoder for three datasets. The orange surfaces represent the manifolds learned by the model, while the blue points correspond to the training data. Each manifold provides a convincing low-dimensional representation of the data, isometric to its respective latent space.
%     }
%     \label{fig:learned_charts}
% \end{figure}

\begin{figure}[htb]
    \centering

    % First row: Projections of RAE for three datasets
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{"results/visualisations/RAE/projections/sinusoid_1_100/more_transparent/5_59_92.jpg"}
        \caption{Dims (5, 59, 92)}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{"results/visualisations/RAE/projections/sinusoid_1_100/more_transparent/31_55_66.jpg"}
        \caption{Dims (31, 55, 66)}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=0.7\textwidth]{"results/visualisations/RAE/projections/sinusoid_1_100/more_transparent/64_72_90.jpg"}
        \caption{Dims (64, 72, 90)}
    \end{subfigure}

    \caption{
        Approximate data manifold learned by the Riemannian autoencoder for the Sinusoid(1, 100) dataset. The orange curves depict the manifold learned by the model, while the blue points show the training data. We visualize three different combinations of the ambient dimensions. %to illustrate how the 1-dimensional manifold is embedded in the higher-dimensional ambient space.
    }
    \label{fig:learned_charts_for_Sinusoid_1_100}
\end{figure}




\subsubsection{Higher-dimensional manifolds}




To evaluate the scalability of our method to higher-dimensional manifolds, we conducted additional experiments on the Hemisphere(5,20) and Sinusoid(5,20) datasets. 

Our theory suggests that the learned variances indicate the importance of each latent dimension: higher variances signal more important dimensions for reconstructing the manifold, while dimensions with vanishing variances are considered insignificant and are disregarded when constructing the Riemannian autoencoder. To test the model's ability to correctly identify important and unimportant latent dimensions, we report the average $\ell^2$ reconstruction error for each dataset as a function of the number of latent dimensions used. In the reconstruction error plots (see \cref{fig:hemisphere_reconstruction_errors,fig:sinusoid_reconstruction_errors}), we report three variance-based orders for adding latent dimensions: decreasing variance order (blue line), increasing variance order (green line), and random order (red line).

For the Hemisphere(5,20) dataset, the model identified five non-vanishing variances (see \cref{fig:hemisphere_variances}), perfectly capturing the intrinsic dimension of the manifold. This is reflected in the blue curve in \cref{fig:hemisphere_reconstruction_errors}, where the first five latent dimensions, corresponding to the largest variances, are sufficient to reduce the reconstruction error almost to zero. In contrast, the green curve illustrates that the remaining ambient dimensions do not encode useful information about the manifold. The red curve demonstrates improvement only when an important latent dimension is included.

For the more challenging Sinusoid(5,20) dataset, our method still performs very well, though not as perfectly as for the Hemisphere dataset. The first six most important latent dimensions explain approximately $97\%$ of the variance, increasing to over $99\%$ with the seventh dimension (see \cref{fig:sinusoid_variances}). This is reflected in the blue curve in \cref{fig:sinusoid_reconstruction_errors}, where the first six latent dimensions reduce the reconstruction error to near zero, and the addition of the seventh dimension brings the error effectively to zero. The slight discrepancy between our results and the ground truth likely arises from increased optimization difficulty, as the normalizing flow must learn a more intricate distribution while maintaining approximate isometry. We believe that with deeper architectures and more careful tuning of the optimization loss, the model will converge to the correct intrinsic dimensionality of five. Currently, it predicts six dimensions at a threshold of $\epsilon = 0.05$ and seven at $\epsilon = 0.01$, slightly overestimating due to the manifold's complexity.


\begin{figure}[t!]
\vspace{-0.5cm}
    \centering
    % Title for Hemisphere
    \textbf{Hemisphere (5,20)} \par\medskip
    
    % First row: Hemisphere plots
    \begin{subfigure}[b]{0.443\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{"results/visualisations/RAE/reconstruction/hemisphere_5_20/diagonal_values_normal_scale.png"}
        \caption{Learned variances in decreasing order.}
        \label{fig:hemisphere_variances}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.546\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{"results/visualisations/RAE/reconstruction/hemisphere_5_20/reconstruction_error_plot_normal_scale.png"}
        \caption{Reconstruction error for three latent orders.}
        \label{fig:hemisphere_reconstruction_errors}
    \end{subfigure}
    
    \vspace{1.5em} % Add some space between the rows
    
    % Title for Sinusoid
    \textbf{Sinusoid (5,20)} \par\medskip
    
    % Second row: Sinusoid plots
    \begin{subfigure}[b]{0.440\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{"results/visualisations/RAE/reconstruction/sinusoid_5_20/diagonal_values_normal_scale.png"}
        \caption{Learned variances in decreasing order.}
        \label{fig:sinusoid_variances}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.549\textwidth}
        \centering
        \includegraphics[width=0.9\textwidth]{"results/visualisations/RAE/reconstruction/sinusoid_5_20/reconstruction_error_plot_normal_scale.png"}
        \caption{Reconstruction error for three latent orders.}
        \label{fig:sinusoid_reconstruction_errors}
    \end{subfigure}

    % Main caption for the entire figure
    \caption{Learned variances and reconstruction errors for the Hemisphere(5,20) and Sinusoid(5,20) datasets. The plots in the left column show the learned variances in decreasing order for each dataset, while the right column illustrates the average $\ell^2$ reconstruction error as a function of the number of latent dimensions used. The reconstruction errors are evaluated for three variance-based orders of the latent dimensions: the \textbf{blue line} (circular markers) represents adding dimensions in decreasing order of variance, the \textbf{green line} (square markers) for increasing variance, and the \textbf{red line} (diamond markers) for a random order.
    % \vspace{-2em}
}

    \label{fig:combined_plot}
\end{figure}









==> sections/A0-proofs-basic-setup.tex <==
\section{Proof of \cref{thm:pull-back-mappings} and an additional result}
\label{app:proof-of-basic-setup}

\begin{proof}[Proof of \cref{thm:pull-back-mappings}]
    First note that $\nabla \stroco \circ \diffeo$ is a diffeomorphism with inverse $\diffeo^{-1} \circ \nabla \stroco^\star$. Then, equations \cref{eq:thm-geodesic-remetrized,eq:thm-log-remetrized,eq:thm-exp-remetrized,eq:thm-distance-remetrized} follow directly from \citep[Prop.~2.1]{diepeveen2024pulling} and \cref{eq:stroco-diffeo-barycentre-formal} follows directly from \citep[Cor.~3.6.1]{diepeveen2024pulling}.

    Next, if $\stroco$ is of the form \cref{eq:quadratic-stroco}, i.e., 
    $$
        \stroco(\Vector)=\frac{1}{2} \Vector^{\top} \spdMatrix^{-1} \Vector,
        % \label{eq:quadratic-stroco}
    $$
    we have that its Fenchel conjugate is given by
    \begin{equation}
        \stroco^\star(\VectorB)=\frac{1}{2} \VectorB^{\top} \spdMatrix \VectorB.
        % \label{eq:quadratic-stroco}
    \end{equation}
    So both $\nabla \stroco(\Vector) = \spdMatrix^{-1} \Vector$ and $\nabla \stroco^\star(\VectorB) = \spdMatrix \VectorB$ are linear mappings, from which follows that they cancel to identity everywhere and yield \cref{eq:thm-geodesic-remetrized-special-psi,eq:thm-log-remetrized-special-psi,eq:thm-exp-remetrized-special-psi,eq:thm-distance-remetrized-special-psi,eq:diffeo-barycentre-formal}.
\end{proof}

\begin{proposition}
    Let $\diffeo:\Real^\dimInd \to \Real^\dimInd$ be a smooth diffeomorphism and let $\stroco: \Real^\dimInd \to \Real$ be a smooth strongly convex function, whose Fenchel conjugate is denoted by $\stroco^\star: \Real^\dimInd\to\Real$. Next, consider the function $f:\Real^\dimInd \to \Real^{\dimInd \times \dimInd}$ given by 
    \begin{equation}
        f(\VectorC) := D_{\VectorC} \nabla \stroco^\star  + \sum_{\sumIndA=1}^\dimInd \VectorC_\sumIndA \partial_\sumIndA D_{(\cdot)} \nabla \stroco^\star.
    \end{equation}
    Finally, let $\Vector, \VectorB \in \Real^\dimInd$ be vectors and assume that for all vectors 
    $$
    \VectorC\in \{(1 - t)(\nabla \stroco \circ \diffeo)(\Vector) + t (\nabla \stroco \circ \diffeo)(\VectorB) \mid t \in [0,1]\} \subset \Real^\dimInd
    $$
    the matrix $f(\VectorC)$ is positive definite.
    
    Then, mapping 
    \begin{equation}
        t \mapsto \stroco(\diffeo(\geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t))), \quad t \in [0,1]
        \label{eq:mapping-conexity-theorem}
    \end{equation}
    is strongly convex, where $\geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}$ is the geodesic between $\Vector$ and $\VectorB$ under the Riemannian structure $(\Real^\dimInd, (\cdot,\cdot)^{\nabla \stroco \circ \diffeo})$. 
    
    In addition, if $\stroco$ is of the form \cref{eq:quadratic-stroco} the mapping \cref{eq:mapping-conexity-theorem} is strongly convex for any $\Vector, \VectorB \in \Real^\dimInd$.
\end{proposition}

\begin{proof}
    By \cref{eq:thm-geodesic-remetrized} in \cref{thm:pull-back-mappings} we have
    \begin{multline}
        \stroco(\diffeo(\geodesic^{\nabla \stroco \circ \diffeo}_{\Vector, \VectorB}(t))) = \stroco(\diffeo((\diffeo^{-1} \circ\nabla \stroco^\star) ((1 - t)(\nabla \stroco \circ \diffeo)(\Vector) + t (\nabla \stroco \circ \diffeo)(\VectorB))))\\
        = \stroco(\nabla \stroco^\star((1 - t)(\nabla \stroco \circ \diffeo)(\Vector) + t (\nabla \stroco \circ \diffeo)(\VectorB))).
    \end{multline}
    So the claim holds if on the linear subspace
    \begin{equation}
        \{(1 - t)(\nabla \stroco \circ \diffeo)(\Vector) + t (\nabla \stroco \circ \diffeo)(\VectorB) \mid t \in [0,1]\} \subset \Real^\dimInd
        \label{eq:subapace-thm-strong-convexity}
    \end{equation}
    the function $\stroco \circ \nabla \stroco^\star$ is convex. 

    Next, note that the Hessian of $\stroco \circ \nabla \stroco^\star$ satisfies
    \begin{equation}
        D_\VectorC \nabla (\stroco \circ \nabla \stroco^\star) = f(\VectorC).
    \end{equation}
    By assumption $f(\VectorC)$ is positive definite for all $\VectorC$ in the subspace \cref{eq:subapace-thm-strong-convexity}. In other words, on this subspace $\stroco(\nabla \stroco^\star(\VectorC))$ is positive definite, which implies strong convexity and yields the main claim.  

    The claim for the special case of $\stroco$ is of the form \cref{eq:quadratic-stroco} follows directly, because
    \begin{equation}
        f(\VectorC) = \spdMatrix,
    \end{equation}
    which is always positive definite.
    
\end{proof}

==> sections/A2-Metric_choices.tex <==
\section{Justifications}
Over the last few decades people have been extending various existing data analysis frameworks to extend to generic Riemannian manifolds, thus improving their universality. Often-times the geometry of the problem is completely pre-specifed, for example climate evolution inherently operates on a sphere. 

The problem of interest for us is the opposite. Instead of using the riemannian geometry to help with data-driven tasks. We hope to extract the riemannian geometry out of data directly, to be used in downstream tasks

\subsection{Discussion of choice of metric and connection to existing work}\label{app:metric_choices}
In connecting with existing work I am hoping we may be able to justify our choice of metric. However, even motivated, there remain many different choices for what the extracted metric could be. Particularly, taking a closer look at what the metric tensor is in \Cref{eq:met_defn}. Particularly, expanding this in coordinates, we get that (using einstein summation convention)
\[
g_{ij} = \nabla_i s_k(x)\nabla_j s_k(x)
\]
Now, if $s(x)$ is a diffeomorphism - this becomes well - justified, as this becomes simply the pullback metric under this diffeo. However, there remain two other choices, which may be more suitable when $s$ is not a diffeomorphism. For this reason I am slightly unsure why we may not be using those? These are:
\[
g^{(1)}_{ij} = s_i(x)s_j(x)
\]
This is directly in analogy with fisher-rao, except here it is the stein score. I also think this is the metric we would want if we were moving on constant likelihood surfaces. I presume this is not what we desire. So realistically we are (should) be comparing the original choice we had with the hessian choice - both can be seen to give what we want when we are gaussian, but they do have inherent differences. The 
And the second choice is the hessian 
\[
g^{(2)}_{ij} = \nabla_i s_j(x) = \nabla_i \nabla_j i(x)
\]
TODO: 
Analogy with Gauss-Newton vs Newton in optimisation to stand (2) and (0) apart, despite equivalence for gaussians.
Particular example for the exponential family. 
Usefulness of (0) as pullback metric for estimating geodesics and etc.

GMM - normalizing flow\cite{izmailov2020semi}
\subsubsection{Motivation as symmetrised KL divergence of posteriors}
Assume we are given a probability density $p(x)$ and consider $p_1(x) = p(x+\Delta x)$ and $p_2(x) = p(x)$. Consider further gaussian smoothed versions $p_1(x | \theta) = p_1(x+\theta)$ and $p_2(x | \theta) = p_2(x+\theta)$, where the prior $\theta \sim \mathcal{N}(0,\sigma^2 I)$. By Bayes 
\[
p_i(\theta | x) = \frac{p(\theta)p_i(x| \theta)}{p_i(x)}
\]
And we ask the question - what is $D_{KL} (p_1(\cdot|x) \| p_2(\cdot|x))$? As we show below it is: 
\[
D_{KL} (p_1(\cdot|x) \| p_2(\cdot|x)) = D_{KL} (p(\cdot|x) \| p(\cdot|x+\Delta x)) =  \sigma^2 s^{\top}(x)(s(x) - s(x+\Delta x)) + o(\sigma^2)
\]
This implies that the symmetrised version is 
\[
D^{sym}_{KL} (p(\cdot|x) \| p(\cdot|x+\Delta x)) =  \sigma^2 (s(x) - s(x+\Delta x))^{\top}(s(x) - s(x+\Delta x)) + o(\sigma^2) 
= \sigma^2 \sum_{ij} \Delta x_j \Delta x_i \partial_i s_k(x) \partial_j s_k(x) +  o(\sigma^2) 
\]
And therefore, the metric we define can be seen as a distance between infinitesimally smoothed posterior densities?
The proof is basically the following:
\begin{align*}
D_{KL} (p(\cdot|x) \| p(\cdot|x+\Delta x)) &= \int d\theta \frac{p(\theta)}{p(x)}p(x+\theta)\left(\log\frac{p(x+\theta)}{p(x)} - \log\frac{p(x+\Delta x+ \theta)}{p(x+\Delta x)} \right) \\   
&= \int d\theta \frac{p(\theta)}{p(x)}\left(p(x)+\theta^\top s(x)p(x)\right)\left(\theta^\top s(x) - \theta^\top s(x+\Delta x)\right) + o(\theta^2) \\
&= \left(s_i(x) -  s_i(x+\Delta x)\right) \int  d\theta p(\theta) \theta_i \\& \qquad + s_j(x) \left(s_i(x) -  s_i(x+\Delta x)\right) \int d\theta p(\theta) \theta_i\theta_j  + o(\theta^2) \\
&= \sigma^2 s_j(x) \left(s_i(x) -  s_i(x+\Delta x)\right)  + o(\sigma^2)
\end{align*}
Therefore the result we may want to prove formally is (probably some assumption on moments and regularity of $p$ is needed. 
\begin{proposition}
Under some regularity conditions
\[
\frac{1}{\sigma^2}D_{J}\left(p(\cdot|x) \| p(\cdot|x+\Delta x)\right) \to 
\|s(x+\Delta x) - s(x)\|^2\text{  as }\sigma \to 0
\]
And this turns into the pullback distance. 
\end{proposition}
This can also directly relate to Tweedies identity. Denoising posterior metric?




==> sections/A7-MNIST.tex <==
\section{Experiments with More Complex Distributions}
\label{app:Experiments-with-more-complex-distributions}

We applied our training framework\footnote{with the minor change of replacing the isometry regularizer to a more scalable version (see \Cref{app:complexity-training} for details)} to model complex real-world and synthetic distributions, specifically focusing on the subset of digit \say{1} from the MNIST dataset and a synthetic dataset of 10-dimensional Gaussian blobs introduced in \citet{stanczuk2022your}. The subset of digit \say{1} is chosen as it is likely to be represented well by the unimodal parametric family \ref{eq:stroco-diffeo-density}. The Gaussian blobs dataset is included because its intrinsic dimension is known (10), providing a reliable baseline for evaluating the accuracy of the RAE’s intrinsic dimension estimation.

Modeling such distributions effectively requires more expressive normalizing flow architectures, such as affine coupling flows combined with \(1 \times 1\) invertible convolutions for pixel reshuffling, or rational quadratic (RQ) spline flows. These architectures, however, are not guaranteed to have zero second derivatives, which can cause the higher-order terms in Theorem~\ref{thm:rae-error} to become significant, potentially inflating the expected reconstruction error of the Riemannian Auto-encoder (RAE). Furthermore, enforcing \(\ell^2\) isometry regularization becomes more challenging in these cases.

Despite these issues, our experiments indicate that the deviations from isometry and the presence of non-zero second derivatives do not visibly impact the quality of the manifold mappings. However, they can affect the overall performance of the RAE.

We trained two models on the digit \say{1} subset of MNIST: an affine coupling flow with \(1 \times 1\) invertible convolution layers (which is not an affine transformation) and an RQ spline flow. In both cases, we observed stable and accurate geodesics that traversed regions of high data density, consistent with theoretical predictions. These geodesics effectively navigate through common examples of the digit \say{1}, as expected based on the learned data distribution. The results are presented in Figure~\ref{fig:mnist_geodesics}.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{results/mnist/affine_mnist_geodesics.png}
        \caption{Affine Coupling Model}
        \label{fig:affine_mnist_geodesics}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{results/mnist/nsf_mnist_geodesics.png}
        \caption{Rational Quadratic Spline Model}
        \label{fig:rqs_mnist_geodesics}
    \end{subfigure}
    \caption{Geodesics computed for two different normalizing flow models trained on the subset of digit \say{1} from the MNIST dataset. (a) shows the geodesics for a model using affine coupling layers with \(1 \times 1\) convolutions, while (b) shows the geodesics for a model using rational quadratic splines. In both cases, the geodesics pass through high-density regions of the dataset, consistent with the theoretical expectation that geodesics align with areas of higher probability under the learned data distribution. This highlights the models' ability to capture the underlying data manifold effectively.}
    \label{fig:mnist_geodesics}
\end{figure}

To complement the MNIST experiments, we evaluated the same models on the Gaussian blobs dataset, where the true intrinsic dimension is known to be 10. This dataset allows us to directly assess the accuracy of the RAE’s intrinsic dimension estimation. The trained affine and RQ spline models produced stable and accurate geodesics similar to those observed in the MNIST experiments, as shown in Figure~\ref{fig:blobs_geodesics}. However, both models overestimated the intrinsic dimension.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{results/blobs/affine_blobs_interpolation.png}
        \caption{Affine Coupling Model}
        \label{fig:affine_blobs_interpolation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{results/blobs/rq_blobs_interpolation.png}
        \caption{Rational Quadratic Spline Model}
        \label{fig:rq_blobs_interpolation}
    \end{subfigure}
    \caption{Geodesics computed for two different normalizing flow models trained on the 10-dimensional Gaussian blobs dataset. (a) shows the geodesics for a model using affine coupling layers with \(1 \times 1\) convolutions, while (b) shows the geodesics for a model using rational quadratic splines. Both models demonstrate smooth geodesics that traverse high-density regions.}
    \label{fig:blobs_geodesics}
\end{figure}

Our RAE model consistently overestimates the intrinsic dimension across both datasets. For the MNIST subset, we observe an estimated intrinsic dimension of approximately 650 for the RQ spline flow and around 300 for the affine flow when using an \(\epsilon = 0.1\) threshold. Similarly, for the Gaussian blobs dataset, the affine model estimates an intrinsic dimension of 650, while the RQ spline model estimates 396. We attribute this overestimation primarily to the difficulty of achieving an \(\ell^2\) isometry while learning the complex data distribution. Although non-zero second derivatives are a secondary factor, they may exacerbate the issue by increasing the contributions of higher-order terms in Theorem~\ref{thm:rae-error}.

These results suggest that while our method can effectively capture the manifold structure, additional regularization may be required to better align the learned metric with the true geometry, especially when using highly expressive flow architectures.


==> sections/A8-computational-complexity.tex <==
\section{Computational complexity of the proposed approach to training}
\label{app:complexity-training}

In this paper we have claimed that this approach is more scalable than the work by \cite{diepeveen2024pulling}. This is the case for most parts of the proposed loss, except for the isometry regularizer, which is also in the loss by \cite{diepeveen2024pulling}.

In our work, we employed the \textbf{exact orthogonal regularization}, which comes down to computing

\[\frac{1}{b} \sum_{\sumIndA=1}^b
\|  (D_{\Vector^\sumIndA} \diffeo_{\networkParams_2})^\top D_{\Vector^\sumIndA} \diffeo_{\networkParams_2}  - \mathbf{I}_\dimInd\|_F^2,
\]

where $b$ is the batch size.

\paragraph{Computational Complexity}

The complexity of the exact method is:

\[
O(b \times d^3 + b \times d \times f),
\]

where:
\begin{itemize}
    \item $d$ is the ambient dimension,
    \item $f$ is the cost of a forward and backward pass through $\diffeo$.
\end{itemize}

This scales \textbf{cubically with $d$} and is \textbf{independent of the intrinsic dimension}. We leveraged PyTorch’s \texttt{vmap} to efficiently compute this for dimensions up to $d = 100$ in our experiments.

\paragraph{Approximate Method for Higher Dimensions}

In the experiments for higher-dimensional data (in \cref{app:Experiments-with-more-complex-distributions}), we used an \textbf{approximate regularization method}. Instead of computing the full Jacobian, we approximate the orthogonality condition using $v$ random orthonormal vectors $\{\mathbf{v}^j\}_{j=1}^{v}$. The regularization term is

\[
\frac{1}{b} \sum_{i=1}^{b} \sum_{j,k=1}^{v} ( (D_{\Vector^\sumIndA} \diffeo_{\networkParams_2}[\mathbf{v}^j])^\top D_{\Vector^\sumIndA} \diffeo_{\networkParams_2} [\mathbf{v}^k] - (\mathbf{I}_v)_{j,k} )^2.
\]
% \todo{@Georgios, in the rebuttal you say that we only use the Jacobian and not the transpose... This is not the same relaxation. It's a lot stronger.}

% where $D_{\Vector^\sumIndA} \diffeo_{\networkParams_2} [\mathbf{v}^j]$ is the Jacobian-vector product for sample $i$ and vector $\mathbf{v}^j$.

\paragraph{Complexity of Approximate Method}

\[
O(b \times d \times v^2 + b \times v \times f + b \times v^3).
\]

This reduces the computational cost, scaling \textbf{linearly with $d$}, and is also independent of the intrinsic dimension. It offers a scalable alternative for high-dimensional datasets. For our main experiments, we used the exact method due to its strong regularization in moderate dimensions ($d \leq 100$). However, the approximate method was tested in preliminary high-dimensional experiments and effectively enforced orthogonality, promoting near-isometric mappings as required by our theoretical framework. The exact method ensures robust regularization in lower to moderate dimensions, while the approximate method provides a scalable alternative for higher-dimensional cases. By leveraging a small number of slicing vectors, it reduces the computational burden while preserving key geometric properties, making it effective across varying dimensional regimes.


==> sections/new_numerics.tex <==
\section{Experiments}
\label{sec:numerics}

We conducted two sets of experiments to evaluate the proposed scheme from \ref{sec:adapting-normalizing-flows} to learn suitable pullback Riemannian geometry. The first set investigates whether our adaptation of the standard normalizing flow (NF) training paradigm leads to more accurate and stable manifold mappings, as measured by the geodesic and variation errors. The second set assesses the capability of our method to generate a robust Riemannian autoencoder (RAE).

For all experiments in this section, detailed training configurations are provided in \ref{app:training_details}.

\subsection{Manifold mappings}
\label{sec:manifold-mappings-experiments}

As discussed in \cite{diepeveen2024pulling}, the quality of learned manifold mappings is determined by two key metrics: the \emph{geodesic error} and the \emph{variation error}. The geodesic error measures the average deviation form the ground truth geodesics implied by the ground truth pullback metric, while the variation error evaluates the stability of geodesics under small perturbations. We define these error metrics for the evaluation of pullback geometries in Appendix \ref{app:Error metrics for evaluation of Pullback Geometries}.

Our approach introduces two key modifications to the normalizing flow (NF) training framework:

\begin{enumerate}
    \item \textbf{Anisotropic Base Distribution}: We parameterize the diagonal elements of the covariance matrix \(\spdMatrix_{\networkParams_1}\), introducing anisotropy into the base distribution.
    
    \item \textbf{\(\ell^2\)-Isometry Regularization}: We regularize the flow \(\diffeo_{\networkParams_2}\) to be approximately \(\ell^2\)-isometric.
\end{enumerate}

To assess the effectiveness of these modifications in learning more accurate and robust manifold mappings, we compare our method against three baselines:

\begin{enumerate}[label=(\arabic*)]
    \item \emph{Normalizing Flow (NF)}: Uses an NF with a standard isotropic Gaussian base distribution $\mathcal{N}(\mathbf{0}, \mathbf{I}_\dimInd)$ and no isometry regularization of the flow.
    \item \emph{Anisotropic Normalizing Flow}: Uses an NF with the same parameterization of the diagonal covariance matrix in the base distribution as in our method, but without regularization of the flow.
    \item \emph{Isometric Normalizing Flow}: Uses an NF with an isotropic Gaussian base distribution $\mathcal{N}(\mathbf{0}, \mathbf{I}_\dimInd)$ and regularizes the flow to be approximately $\ell^2$-isometric.
\end{enumerate}

We conduct experiments on three datasets, illustrated in \ref{fig:datasets} in \ref{app:manifold_mapping}: the \emph{Single Banana Dataset}, the \emph{Squeezed Single Banana Dataset}, and the \emph{River Dataset}. Detailed descriptions of the construction and characteristics of these datasets are provided in \ref{app:manifold_mapping}.

\cref{tab:geodesic-variation-errors} presents the geodesic and variation errors for each method across the three datasets and \cref{fig:geodesics_comparison} visually compares the geodesics computed using each method on the river dataset. Our method consistently achieves significantly lower errors compared to the baselines, indicating more accurate and stable manifold mappings. 

Introducing anisotropy in the base distribution without enforcing isometry in the flow offers no significant improvement over the standard flow. On the other hand, regularizing the flow to be approximately isometric without incorporating anisotropy in the base distribution results in underfitting, leading to noticeably worse performance than the standard flow. Our results demonstrate that the combination of anisotropy in the base distribution with isometry regularization (our method) yields the most accurate and stable manifold mappings, as evidenced by consistently lower geodesic and variation errors.

\begin{table*}[t!]
    \centering
    \begin{tabular}{lcccc}
    \hline
    \textbf{Metric} & \textbf{Our Method} & \textbf{NF} & \textbf{Anisotropic NF} & \textbf{Isometric NF} \\
    \hline
    \multicolumn{5}{c}{\textbf{Single Banana Dataset}} \\
    \hline
    Geodesic Error & \textbf{0.0315 (0.0268)} & 0.0406 (0.0288) & 0.0431 (0.0305) & 0.0817 (0.1063) \\
    Variation Error & \textbf{0.0625 (0.0337)} & 0.0638 (0.0352) & 0.0639 (0.0354) & 0.0639 (0.0355) \\
    \hline
    \multicolumn{5}{c}{\textbf{Squeezed Single Banana Dataset}} \\
    \hline
    Geodesic Error & \textbf{0.0180 (0.0226)} & 0.0524 (0.0805) & 0.0505 (0.0787) & 0.1967 (0.2457) \\
    Variation Error & \textbf{0.0631 (0.0326)} & 0.0663 (0.0353) & 0.0661 (0.0350) & 0.0669 (0.0361) \\
    \hline
    \multicolumn{5}{c}{\textbf{River Dataset}} \\
    \hline
    Geodesic Error & \textbf{0.1691 (0.0978)} & 0.2369 (0.1216) & 0.2561 (0.1338) & 0.3859 (0.2568) \\
    Variation Error & \textbf{0.0763 (0.0486)} & 0.1064 (0.0807) & 0.1113 (0.0863) & 0.0636 (0.0333) \\
    \hline
    \end{tabular}
    \caption{Comparison of evaluation metrics for different methods across three datasets. Best-performing results for each metric are highlighted in bold. Values are reported as mean (std). The proposed method performs best in all metrics on each data set.}
    \label{tab:geodesic-variation-errors}
    \end{table*}

    \begin{figure*}[htbp]
        \centering
        \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\textwidth]{results/visualisations/geodesics/gt.png}
        \caption{\scriptsize Ground Truth}
        \end{subfigure}
        \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\textwidth]{results/visualisations/geodesics/ours.png}
        \caption{\scriptsize Our Method}
        \end{subfigure}
        \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\textwidth]{results/visualisations/geodesics/standard_normal.png}
        \caption{\scriptsize Standard NF}
        \end{subfigure}
        \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\textwidth]{results/visualisations/geodesics/standard_normal_anisotropic.png}
        \caption{\scriptsize Anisotropic NF}
        \end{subfigure}
        \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\textwidth]{results/visualisations/geodesics/isometricNF.png}
        \caption{\scriptsize Isometric NF}
        \end{subfigure}
        \caption{Comparison of geodesics computed using different methods on the river dataset. The geodesics generated by the proposed method have the fewest artifacts, aligning with expectations from Table~\ref{tab:geodesic-variation-errors}.}
        \label{fig:geodesics_comparison}
    \end{figure*}
    

\subsection{Riemannian Autoencoder}\label{sec:RAE-experiments}
    
    To evaluate the ability of our method to learn a Riemannian autoencoder, we conducted experiments on synthetic and real-world datasets:

    \begin{itemize} \item \textit{Hemisphere}($\dimInd'$, $\dimInd$) and \textit{Sinusoid}($\dimInd'$, $\dimInd$): Synthetic datasets with controllable intrinsic dimension $\dimInd'$ and ambient dimension $\dimInd$. \item $\dimInd'$-\textit{Gaussian Blobs Image Manifold}: A synthetic image dataset with controllable intrinsic dimension $\dimInd'$ embedded in a 1024-dimensional ambient space. \item \textit{MNIST}: Experiments were conducted on the digit \say{1} subset and the full dataset of handwritten digits, both embedded in a 1024-dimensional ambient space. \end{itemize}
    
    \noindent For a detailed description of these datasets, refer to \ref{app:rae_datasets}.

    \subsubsection{1D and 2D manifolds}
    In \cref{fig:learned_charts,fig:learned_charts_for_Sinusoid_1_100}, we present the data manifold approximations by our Riemannian autoencoder for four low-dimensional manifolds.: Hemisphere(2,3), Sinusoid(1,3), Sinusoid(2,3) and Sinusoid(1,100). In \ref{app:data_manifold_approximation}, we detail the process used to create the data manifold approximations for these experiments. In our experiments, we set \( \epsilon = 0.01 \), which resulted in \( d_{\epsilon} = \dimInd' \) for all cases, accurately capturing the intrinsic dimension of each manifold and producing accurate global charts.

    \begin{figure*}[htb]
        \centering
    
        % First row: Projections of RAE for three datasets
        \begin{subfigure}[b]{0.32\textwidth}
            \centering
            \includegraphics[width=\textwidth]{results/visualisations/RAE/projections/sinusoid_1_100/more_transparent/5_59_92.jpg}
            \caption{Dims (5, 59, 92)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\textwidth}
            \centering
            \includegraphics[width=\textwidth]{results/visualisations/RAE/projections/sinusoid_1_100/more_transparent/31_55_66.jpg}
            \caption{Dims (31, 55, 66)}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.32\textwidth}
            \centering
            \includegraphics[width=\textwidth]{results/visualisations/RAE/projections/sinusoid_1_100/more_transparent/64_72_90.jpg}
            \caption{Dims (64, 72, 90)}
        \end{subfigure}
    
        \caption{
            Approximate data manifold learned by the Riemannian autoencoder for the Sinusoid(1, 100) dataset. The orange curves depict the manifold learned by the model, while the blue points show the training data. We visualize three different combinations of the ambient dimensions. %to illustrate how the 1-dimensional manifold is embedded in the higher-dimensional ambient space.
        }
        \label{fig:learned_charts_for_Sinusoid_1_100}
    \end{figure*}


\subsubsection{Higher-dimensional manifolds}



    \begin{figure*}[h!]
        % \vspace{-0.5cm}
            \centering
            % Title for Hemisphere
            \textbf{Hemisphere (5,20)} \par\medskip
            
            % First row: Hemisphere plots
            \begin{subfigure}[b]{0.443\textwidth}
                \centering
                \includegraphics[width=\textwidth]{results/visualisations/RAE/reconstruction/hemisphere_5_20/diagonal_values_normal_scale.png}
                \caption{Learned variances in decreasing order.}
                \label{fig:hemisphere_variances}
            \end{subfigure}
            \hfill
            \begin{subfigure}[b]{0.546\textwidth}
                \centering
                \includegraphics[width=\textwidth]{results/visualisations/RAE/reconstruction/hemisphere_5_20/reconstruction_error_plot_normal_scale.png}
                \caption{Reconstruction error for three latent orders.}
                \label{fig:hemisphere_reconstruction_errors}
            \end{subfigure}
            
            \vspace{1.5em} % Add some space between the rows
            
            % Title for Sinusoid
            \textbf{Sinusoid (5,20)} \par\medskip
            
            % Second row: Sinusoid plots
            \begin{subfigure}[b]{0.440\textwidth}
                \centering
                \includegraphics[width=\textwidth]{results/visualisations/RAE/reconstruction/sinusoid_5_20/diagonal_values_normal_scale.png}
                \caption{Learned variances in decreasing order.}
                \label{fig:sinusoid_variances}
            \end{subfigure}
            \hfill
            \begin{subfigure}[b]{0.549\textwidth}
                \centering
                \includegraphics[width=\textwidth]{results/visualisations/RAE/reconstruction/sinusoid_5_20/reconstruction_error_plot_normal_scale.png}
                \caption{Reconstruction error for three latent orders.}
                \label{fig:sinusoid_reconstruction_errors}
            \end{subfigure}
        
            % Main caption for the entire figure
            \caption{Learned variances and reconstruction errors for the Hemisphere(5,20) and Sinusoid(5,20) datasets. The plots in the left column show the learned variances in decreasing order for each dataset, while the right column illustrates the average $\ell^2$ reconstruction error as a function of the number of latent dimensions used. The reconstruction errors are evaluated for three variance-based orders of the latent dimensions: the \textbf{blue line} (circular markers) represents adding dimensions in decreasing order of variance, the \textbf{green line} (square markers) for increasing variance, and the \textbf{red line} (diamond markers) for a random order.\vspace{-2em}
        }
        
            \label{fig:combined_plot}
        \end{figure*}

    To evaluate the scalability of our method to higher-dimensional manifolds, we conducted additional experiments on the Hemisphere(5,20) and Sinusoid(5,20) datasets. 
    
    Our theory suggests that the learned variances indicate the importance of each latent dimension: higher variances signal more important dimensions for reconstructing the manifold, while dimensions with vanishing variances are considered insignificant and are disregarded when constructing the Riemannian autoencoder. To test the model's ability to correctly identify important and unimportant latent dimensions, we report the average $\ell^2$ reconstruction error for each dataset as a function of the number of latent dimensions used. In the reconstruction error plots (see \ref{fig:hemisphere_reconstruction_errors},\ref{fig:sinusoid_reconstruction_errors}), we report three variance-based orders for adding latent dimensions: decreasing variance order (blue line), increasing variance order (green line), and random order (red line).
    
    For the Hemisphere(5,20) dataset, the model identified five non-vanishing variances (see \ref{fig:hemisphere_variances}), perfectly capturing the intrinsic dimension of the manifold. This is reflected in the blue curve in \ref{fig:hemisphere_reconstruction_errors}, where the first five latent dimensions, corresponding to the largest variances, are sufficient to reduce the reconstruction error almost to zero. In contrast, the green curve illustrates that the remaining ambient dimensions do not encode useful information about the manifold. The red curve demonstrates improvement only when an important latent dimension is included.
    
    For the more challenging Sinusoid(5,20) dataset, our method still performs very well, though not as perfectly as for the Hemisphere dataset. The first six most important latent dimensions explain approximately $97\%$ of the variance, increasing to over $99\%$ with the seventh dimension (see \ref{fig:sinusoid_variances}). This is reflected in the blue curve in \ref{fig:sinusoid_reconstruction_errors}, where the first six latent dimensions reduce the reconstruction error to near zero, and the addition of the seventh dimension brings the error effectively to zero. The slight discrepancy between our results and the ground truth likely arises from increased optimization difficulty, as the normalizing flow must learn a more intricate distribution while maintaining approximate isometry. We believe that with deeper architectures and more careful tuning of the optimization loss, the model will converge to the correct intrinsic dimensionality of five. Currently, it predicts six dimensions at a threshold of $\epsilon = 0.05$ and seven at $\epsilon = 0.01$, slightly overestimating due to the manifold's complexity.
    
    \subsubsection{Image Experiments}
    \begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{results/blobs/variance_and_reconstruction.png}
    \caption{Cumulative normalized variances (top) and reconstruction errors (bottom) for $d'$-Gaussian Blobs across different settings (20, 50, 100).}
    \label{fig:variance_reconstruction}
\end{figure}




    \label{sec:mnist_experiments}
    \begin{figure*}[h!]
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/digit_1_variances.png}
            \caption{\scriptsize Digit ``1'': Variances.}
        \end{subfigure}
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/all_digits_variances.png}
            \caption{\scriptsize All digits: Variances.}
        \end{subfigure}
        \caption{Learned latent variances on MNIST digit ``1'' and all digits. Using $\epsilon = 0.1$, we detect 127 latent dimensions for digit ``1'' and 176 for all digits.}
        \label{fig:mnist_variances}
    \end{figure*}

    
    To evaluate the RAE on real-world data, we conducted experiments on the MNIST dataset, considering two settings: (i) using only the digit ``1'' subset and (ii) using the full dataset with all digits. Initially, we used the same loss in \eqref{eq:basic_training_objective} as in previous experiments, regularizing $\diffeo_{\networkParams_2}$ for isometry and volume preservation. While geodesic interpolations worked well, the RAE's intrinsic dimension estimate was poor. For instance, in the digit ``1'' subset, the RAE predicted roughly 400 latent dimensions, far exceeding the ID-DIFF \cite{pmlr-v235-stanczuk24a} estimate of 66.
    
    Upon further investigation (Appendix~\ref{app:expanded_loss_function}), we identified a Hessian vector product term in the model’s log-density that can disrupt the assignment of large variances to important latent dimensions. In all other experiments presented above, this term was effectively zero because $\diffeo_{\networkParams_2}$ was purely affine (composition of affine coupling layers only). For MNIST, we included $1 \times 1$ invertible convolutions after each affine coupling layer for channel mixing, making $\diffeo_{\networkParams_2}$ non-affine and potentially introducing significant second-order terms.
    
    \begin{figure*}[h!]
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/digit_1_original.png}
            \caption{\scriptsize Digit ``1'': Original.}
        \end{subfigure}
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/digit_1_reconstruction.png}
            \caption{\scriptsize Digit ``1'': Reconstruction.}
        \end{subfigure}
        \\
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/all_digits_original.png}
            \caption{\scriptsize All digits: Original.}
        \end{subfigure}
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/all_digits_reconstruction.png}
            \caption{\scriptsize All digits: Reconstruction.}
        \end{subfigure}
        \caption{Original vs.\ reconstructed images on the MNIST digit ``1'' (using 127 latent dimensions) and all digits (using 176 latent dimensions). Reconstructions are mostly accurate with occasional global and local artifacts.}
        \label{fig:mnist_reconstructions}
    \end{figure*}

    Including the Hessian vector product term as an additional regularization term in the loss function, 
    \begin{align}
        \label{eq:mnist_training_objective}
        \mathcal{L}(\theta_1, \theta_2) :=\ & \mathbb{E}_{\stoVector \sim p_{\text{data}}}\bigl[-\log p_{\theta_1, \theta_2}(\stoVector)\bigr] \notag \\
        & + \lambda_{\text{vol}} \, \mathbb{E}_{\stoVector \sim p_{\text{data}}}\Bigl[\bigl(\log \bigl|\det\bigl(D_{\stoVector}\diffeo_{\networkParams_2}\bigr)\bigr|\bigr)^2\Bigr] \notag \\
        & + \lambda_{\text{iso}} \, \mathbb{E}_{\stoVector \sim p_{\text{data}}}\Bigl[\bigl\|\bigl(D_{\stoVector}\diffeo_{\networkParams_2}\bigr)^\top D_{\stoVector}\diffeo_{\networkParams_2} - \mathbf{I}_d\bigr\|_F^2\Bigr] \notag \\
        & + \lambda_{\text{hess}} \, \mathbb{E}_{\stoVector \sim p_{\text{data}}}\Bigl[\bigl\|D^2_{\stoVector}\diffeo_{\networkParams_2} \cdot \spdMatrix_{\theta_1}^{-1} \diffeo_{\networkParams_2}(\stoVector)\bigr\|_2\Bigr],
    \end{align}
    improved RAE's performance substantially. On digit ``1,'' the estimated dimension fell from 400 to 127, closer to the ID-DIFF estimate of 66. On all digits, the RAE detected dimension 176, near ID-DIFF’s estimate of 152. Figure~\ref{fig:mnist_variances} shows the learned variances for these two cases ($\epsilon = 0.1$ yields 127 and 176 dimensions, respectively). Reconstructions in Figure~\ref{fig:mnist_reconstructions} are mostly good, aside from some artifacts (likely due to numerical instability of affine coupling layers when evaluated in the inverse direction). We expect that using more expressive and numerically stable transforms (e.g., rational quadratic spline flows) could further improve results.
    
    
    
    
    
    \begin{figure*}[htbp]
        \centering
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/digit_1_interpolation.png}
            \caption{\scriptsize Digit ``1'': Interpolation.}
        \end{subfigure}
        \begin{subfigure}[b]{0.45\textwidth}
            \includegraphics[width=\textwidth]{results/mnist/all_digits_interpolation.png}
            \caption{\scriptsize All digits: Interpolation.}
        \end{subfigure}
        \caption{Latent space geodesic interpolations for MNIST digit ``1'' (left) and MNIST all digits (right). Geodesic paths remain on the manifold, transitioning smoothly between endpoints.}
        \label{fig:mnist_interpolations}
    \end{figure*}
    
    Overall, these experiments illustrate that our approach scales to real-world data, provided we incorporate the Hessian vector product regularization term when using non-affine flows. We note that the resulting RAE still tends to overestimate the latent dimension slightly, which could stem from (i) the data distribution’s multimodality, thus deviating from our unimodal assumption, and (ii) the difficulty of learning a distribution with a near-isometric, low-curvature flow. Despite this slight overestimation, the method reliably captures the underlying latent structure, yielding meaningful latent representations and smooth geodesic paths. These results mark significant progress toward robust data-driven Riemannian geometry in high-dimensional settings.


==> sections/score-metric.tex <==
\section{Score-based pullback geometry}
The ultimate goal of data-driven Riemannian geometry is to construct a Riemannian structure such that geodesics pass through the support of the distribution, avoiding (very) low density regions and tending towards high density regions. Unfortunately, there is no unique way to achieve this and proposals in the literature vary significantly in both their computational overheads and data access. For a more in-depth discussion of potential choices for the metric see \Cref{app:metric_choices}.  

In this work, we propose a pullback based metric, resulting in efficient manifold mappings. Given a (parameterized) data distribution $p_{\mathcal{X}}:\Real^\dimInd \to \Real$, consider the tensor field $(\,\cdot\,, \,\cdot\,) \colon \vectorfield(\manifold) \times \vectorfield(\manifold) \to C^\infty(\manifold)$ given by
\begin{equation}\label{eq:met_defn}
    (\tangentVector, \tangentVectorB)_{\Vector} := (D_{\Vector} \nabla \log p (\cdot) [\tangentVector_\Vector], D_{\Vector} \nabla  \log p (\cdot) [\tangentVectorB_\Vector])_2.
\end{equation}
The above tensor field generates a Riemannian structure if the score function $\Vector \mapsto \nabla \log p (\Vector)$ is a diffeomorphism. This, for example, holds in the case of a gaussian $p (\Vector) \propto e^{-\frac{1}{2}\|\Vector\|_2^2}$, giving a scalar multiple of the standard $\ell^2$ inner product. In other words, the data distribution tells us that there is no preferred direction in the data set, in line with our expectations. 

Unlike density based riemannian approaches \cite{sorrenson2024learningdistancesdatanormalizing}, the pullback based metric has an underlying statistical distance interpretation as the noising posterior divergence: 
\begin{proposition}
    Consider $\hat{X} = X + \epsilon$, with $\epsilon\sim\mathcal{N}(0,\sigma^2I)$ and $X\sim p_\mathcal{X}$, then we can consider the noise posterior $p(\epsilon | \hat{X})$, which leads to the desired pullback distance:
    \begin{equation}
        \frac{1}{\sigma^2} D \left(p\left(\cdot|x_1\right) \|\, p\left(\cdot|x_2\right)\right) \to 
\|s(x_1) - s(x_2)\|^2\text{  as }\sigma \to 0
    \end{equation}
\end{proposition}
\todo{zs: Write the nice interpretabilities - of section 4}
% In the case of a unimodal and star shaped -- which is already a non-trivial non-convex case \cite{leong2022optimal} --, there is hope. For general $p$, we do expect more interesting behaviour. That is, if the above tensor field is actually a metric tensor field.

% In practice we don't have the score function, but we can try to obtain an approximation $\score: \Real^\dimInd \to \Real^\dimInd$, which then yields a metric tensor field $(\,\cdot\,, \,\cdot\,)^\score \colon \vectorfield(\manifold) \times \vectorfield(\manifold) \to C^\infty(\manifold)$ given by
% \begin{equation}
%     (\tangentVector, \tangentVectorB)^\score_{\Vector} :=  (D_{\Vector} \score (\cdot) [\tangentVector_\Vector], D_{\Vector} \score (\cdot)[\tangentVectorB_\Vector])_2.
% \end{equation}
% On top of that, it has already been observed that the score is able to tell you properties of the manifold such as the dimension \cite{stanczuk2022your}.

% \paragraph{Finding the score}
% The score can be obtained through training a diffusion model \cite{song2020score}. However, we have to make sure that we get a diffeomorphism, which we can enforce through further assumption, e.g., we can represent the score as
% \begin{equation}
%     \score(\Vector) :=  - \nabla(\stroco \circ \diffeo) (\Vector) = - ((D_{\Vector} \diffeo)^{\top} \circ \nabla\stroco \circ \diffeo) (\Vector),
% \end{equation}
% where $\stroco^\sumIndA:\Real^\dimInd \to \Real$ are strongly convex functions and $\diffeo^\sumIndA:\Real^\dimInd \to \Real^\dimInd$ diffeomorphisms. The score is not per se invertible, because we need information on $\Vector$. Indeed, formally an inverse would look like
% \begin{equation}
%     \score_{\Vector}^{-1}(\VectorB) :=  - (\diffeo^{-1} \circ\nabla \stroco^* \circ (D_{\diffeo(\Vector)} \diffeo^{-1})^\top ) (\VectorB),
% \end{equation}
% where $\stroco^*: \Real^\dimInd \to \Real$ is the Fenchel conjugate of $\stroco$, with $\nabla\stroco^* = (\nabla\stroco)^{-1}$. Then, we do have that $\score_{\Vector}^{-1} (\score(\Vector)) = 
% \Vector$. 


\paragraph{Riemannian geometry of Normalizing Flows}
Since the score is not necessarily invertible, the Riemannian structure does not come with closed-form manifold mappings, zero curvature and symmetry as one hope for \cite{diepeveen2024pulling}. However, with simple regularization, score function of a normalizing flow can be used. To be precise, the score of a normalizing flow in \Cref{eq:nf} is: 
\[
\score(\Vector) = D_{\Vector} \diffeo^{\top} \left[\nabla \log p_\mathcal{Z}\right](\diffeo(\Vector)) + \nabla\log|\operatorname{det}D_{\Vector} \diffeo|
\]
Assuming that $\log p_\mathcal{Z}$ is strongly convex (henceforth denoted as $\psi$), as is the case for a Gaussian target, we can use the pseudo-score
\begin{equation}
    \pseudoscore (\Vector) := (\nabla\stroco \circ \diffeo) (\Vector),
\end{equation}
which gives geometrically the same information as the score as long as $D_{\Vector} \diffeo$ is an orthogonal operator. The pseudo-score is invertible and its inverse is
\begin{equation}
    \pseudoscore^{-1}(\VectorB) :=  (\diffeo^{-1} \circ\nabla \stroco^*) (\VectorB),
\end{equation}
So the metric tensor field $(\,\cdot\,, \,\cdot\,)^{\pseudoscore} \colon \vectorfield(\manifold) \times \vectorfield(\manifold) \to C^\infty(\manifold)$ given by
\begin{equation}
    (\tangentVector, \tangentVectorB)^{\pseudoscore}_{\Vector} :=  (D_{\Vector} \pseudoscore (\cdot) [\tangentVector_\Vector], D_{\Vector} \pseudoscore(\cdot) [\tangentVectorB_\Vector])_2.
\end{equation}
comes with closed-form manifold mappings, with zero curvature and symmetry \cite{diepeveen2024pulling}.
